Statistical Inference for High-Dimensional Matrix-Variate Factor Model

This paper considers the estimation and inference of the low-rank components in high-dimensional matrix-variate factor models, where each dimension of the matrix-variates ($p \times q$) is comparable to or greater than the number of observations ($T$). We propose an estimation method called $\alpha$-PCA that preserves the matrix structure and aggregates mean and contemporary covariance through a hyper-parameter $\alpha$. We develop an inferential theory, establishing consistency, the rate of convergence, and the limiting distributions, under general conditions that allow for correlations across time, rows, or columns of the noise. We show both theoretical and empirical methods of choosing the best $\alpha$, depending on the use-case criteria. Simulation results demonstrate the adequacy of the asymptotic results in approximating the finite sample properties. The $\alpha$-PCA compares favorably with the existing ones. Finally, we illustrate its applications with a real numeric data set and two real image data sets. In all applications, the proposed estimation procedure outperforms previous methods in the power of variance explanation using out-of-sample 10-fold cross-validation.

==> consist-k.tex <==
\subsection{Theorem \ref{thm:consistent-k}: Consistent latent dimension estimators} \label{sec:proof_consistent-k}



\subsubsection{ Behavior of \texorpdfstring{$\lambda_i \paran{\frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top}$}{Lambda i} for \texorpdfstring{$i \le k$}{i <= k}}

Let $\lambda_i$ denote the $i$-th largest eigenvalue of matrix $\bA$ and $\sigma_i$ the $i$-th singular value of $\bA$. Then $\hat{\lambda}_i = \lambda_i \paran{\frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top}$

\begin{lemma} \label{thm:lemma-eigenval-le-k}
    For $i = 1, \cdots, k - 1$,
    \[
    \frac{\hat{\lambda}_{j}}{\hat{\lambda}_{j+1}} = \Op{1}.
    \]
\end{lemma}

\begin{proof}
    The result follows immediate from Proposition \ref{thm:bound V}.
\end{proof}

\subsubsection{ Behavior of \texorpdfstring{$\lambda_i \paran{\frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top}$}{Lambda i} for \texorpdfstring{$i > k$}{i > k} }

\begin{lemma} \label{thm:lemma-eigenval-ge-k},
    For $j = 1, \cdots, p - k$,
    \[
    c + \op{1} \le p \cdot \hat{\lambda}_{k+j} \le C + \op{1},
    \]
    where $c$, $C$, and $\op{1}$ are uniform in $1 \le j \le p - k$.
\end{lemma}

\begin{proof}
    Let $\bX_t = \bF_t \bC^\top$, we decompose
    \[
    \bY_t = \bR \bX_t + \bE_t = \paran{ \bR + \bE_t \bX_t^\top \paran{\bX_t \bX_t^\top}^{-1} } \bX_t + \bE_t \paran{\bI -  \bX_t^\top \paran{\bX_t \bX_t^\top}^{-1} \bX_t}.
    \]
    Then,
    \begin{eqnarray}
        \frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top & = & \paran{ \bR + \bE_t \bX_t^\top \paran{\bX_t \bX_t^\top}^{-1} } \bX_t \bX_t^\top \paran{ \bR + \bE_t \bX_t^\top \paran{\bX_t \bX_t^\top}^{-1} }^\top \nonumber \\
        &   & + \; \bE_t \paran{\bI -  \bX_t^\top \paran{\bX_t \bX_t^\top}^{-1} \bX_t} \bE_t^\top \nonumber
    \end{eqnarray}

    From Weyl inequality and the fact that $\bX_t$ is a $k \times q$ matrix,
    \begin{eqnarray}
        \lambda_{k + j} \paran{ \frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top } & \ge & \lambda_{k + j} \paran{ \frac{1}{p q T} \sum_{t = 1}^{T}  \bE_t \paran{\bI -  \bX_t^\top \paran{\bX_t \bX_t^\top}^{-1} \bX_t} \bE_t^\top } \nonumber \\
        & = & \lambda_{k + j} \paran{ \frac{1}{p q T} \sum_{t = 1}^{T}  \bE_t \paran{\bI -  \bX_t^\top \paran{\bX_t \bX_t^\top}^{-1} \bX_t} \bE_t^\top } \nonumber \\
        & & + \; \lambda_{k + 1} \paran{ \frac{1}{p q T} \sum_{t = 1}^{T}  \bE_t \bX_t^\top \paran{\bX_t \bX_t^\top}^{-1} \bX_t \bE_t^\top } \nonumber \\
        & \ge & \lambda_{2k + j} \paran{ \frac{1}{p q T} \sum_{t = 1}^{T} \bE_t \bE_t^\top}. \nonumber
    \end{eqnarray}

    From Weyl inequality and the fact that $\bX_t$ is a $k \times q$ matrix,
    \begin{eqnarray}
        \lambda_{k + j} \paran{ \frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top } & \le & \lambda_{k + 1} \paran{ \frac{1}{p q T} \sum_{t = 1}^{T} \paran{ \bR + \bE_t \bX_t^\top \paran{\bX_t \bX_t^\top}^{-1} } \bX_t \bX_t^\top \paran{ \bR + \bE_t \bX_t^\top \paran{\bX_t \bX_t^\top}^{-1} }^\top } \nonumber \\
        & & + \; \lambda_j \paran{ \frac{1}{p q T} \sum_{t = 1}^{T} \bE_t \paran{\bI -  \bX_t^\top \paran{\bX_t \bX_t^\top}^{-1} \bX_t} \bE_t^\top }  \nonumber \\
        & \le & \lambda_j \paran{ \frac{1}{p q T} \sum_{t = 1}^{T} \bE_t \paran{\bI -  \bX_t^\top \paran{\bX_t \bX_t^\top}^{-1} \bX_t} \bE_t^\top } \nonumber \\
        & \le & \lambda_j \paran{ \frac{1}{p q T} \sum_{t = 1}^{T} \bE_t \bE_t^\top }. \nonumber
    \end{eqnarray}

    Thus,
    \[
    \lambda_p \paran{ \frac{1}{q T} \sum_{t = 1}^{T} \bE_t \bE_t^\top } \le p \lambda_{k + j} \paran{ \frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top } \le \lambda_1 \paran{ \frac{1}{q T} \sum_{t = 1}^{T} \bE_t \bE_t^\top }
    \]

    From Lemma \ref{thm:EtEt}, we have
    \[
    \norm{ \frac{1}{q T} \sum_{t = 1}^{T} \bE_t \bE_t^\top - \E{\frac{1}{q T} \sum_{t = 1}^{T} \bE_t \bE_t^\top} } = \op{1}.
    \]
    From Condition \ref{assume:cross_row_col_corr_0}.2, the minimal and maximal eigenvalues of $\E{\frac{1}{q T} \sum_{t = 1}^{T} \bE_t \bE_t^\top} $ are bounded away from above and below.
    So we have
    \[
    c + \op{1} \le \lambda_p \paran{ \frac{1}{q T} \sum_{t = 1}^{T} \bE_t \bE_t^\top } \le \lambda_1 \paran{ \frac{1}{q T} \sum_{t = 1}^{T} \bE_t \bE_t^\top} \le C + \op{1} .
    \]
    Finally, we have for $j = 1, \cdots, p - k$,
    \[
    c + \op{1} \le p \cdot \hat{\lambda}_{k+j} \le C + \op{1}.
    \]
\end{proof}

\subsubsection{ Proof of Theorem \ref{thm:consistent-k} }
%\noindent\textbf{Proof of Theorem \ref{thm:consistent-k}}

\begin{proof}
    Let $\Gamma_i \defeq \frac{\hat{\lambda}_{i}}{\hat{\lambda}_{i+1}}$.
    By Lemma \ref{thm:lemma-eigenval-le-k}, we have $\Gamma_i =\Op{1}$ uniformly for $i = 1, \cdots, k-1$.
    We also have $\Gamma_i =\Op{1}$, uniformly for $i = k+1, \cdots, p-1$, since uniformly for $i = k+1, \cdots, p$, $c + \op{1} \le p \cdot \hat{\lambda}_{k+j} \le C + \op{1}$ by Lemma \ref{thm:lemma-eigenval-ge-k}.
    However, when $i = k$,
    \[
    \Gamma_k \ge \tilde c p - \op{1}, \quad \text{ for some } \tilde c > 0.
    \]
    Since $k \le 2p$, we have $p/2 \le p - k - 1$. Define
    \[
    \calI = \braces{i \le p/2: i \ne k}.
    \]
    Then for any $\epsilon > 0$, there is $C > 0$, $\PP \paran{ \underset{i \in \calI}{\max} \; \Gamma_i \ge C } \le \epsilon$.
    Then,
    \begin{eqnarray}
        \PP \paran{\hat k \ne k} & \le & \PP \paran{ \underset{i \in \calI}{\max} \; \Gamma_i \ge \Gamma_k } \nonumber \\
        & \le & \PP \paran{ \underset{i \in \calI}{\max} \; \Gamma_i > C } + \PP \paran{ \Gamma_k \le \underset{i \in \calI}{\max} \; \Gamma_i < C }  \nonumber \\
        & \le & \epsilon. \nonumber
    \end{eqnarray}
    Since $\epsilon$ is arbitrary, we have $\PP \paran{\hat k \ne k} \rightarrow 0$.
\end{proof}

==> misc-proofs-B.tex <==


\paragraph{Proof of Lemma \ref{assume:factor_noise_weak_corr_0}.}

\begin{proof}

    \underline{\sc Step 1.} We first show that
    for any $i \in [p]$,  $j\in[q]$,
    \begin{eqnarray}
        &\E{\norm{\frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, ij}\bF_{t}}^2} = \bigO{1}, \quad
        \E{\norm{\sqrt{\frac{T}{q}} \sum_{j=1}^{q}\bar e_{ij}\bar\bF}^2} = \bigO{1}, \label{eqn:lemma-fn-1} \\
        &\E{\norm{\frac{1}{\sqrt{p T}} \sum_{t=1}^{T} \sum_{i=1}^{p} e_{t, ij}\bF_{t}}^2} = \bigO{1}, \quad
        \E{\norm{\sqrt{\frac{T}{p}} \sum_{i=1}^{p}\bar e_{ij}\bar\bF}^2} = \bigO{1}. \label{eqn:lemma-fn-2}
    \end{eqnarray}

    Proofs for \eqref{eqn:lemma-fn-1} and \eqref{eqn:lemma-fn-2} are the same. Here we only present the proof for \eqref{eqn:lemma-fn-1}.

    For any $i\in[p]$ and $t\in [T]$, we define a random vector $\bx_t = \frac{1}{\sqrt{q}} \sum_{j=1}^q \bC_{j\cdot} e_{t, i j}$, which is $\alpha$-mixing over $t$.
    We rewrite $ \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, ij}\bF_{t} = \frac{1}{\sqrt{T}} \sum_{t=1}^{T} x_t\bF_t$.
    By Assumption \ref{assume:factor-noise-matrix}, we have $\E{x_t\bF_t} = 0$.

    Now we show that there exists some $m > 2$ such that $\EE\norm{x_t \bF_t}^m \le C <\infty$.
    For any $l\in[k]$ and $h\in[r]$,  by Holder inequality, we have for any $1< a, b < \infty$ and $1/a + 1/b = 1$,
    \begin{equation*}
        \E{\abs{ f_{t,lh} x_t}^m}
        = \E{\abs{f_{t,lh}}^m \abs{x_t}^m}
        \le \paran{ \E{\abs{f_{t,lh}}^{ma} } }^{1/a} \paran{\E{\abs{x_t}^{mb}}}^{1/b}.
    \end{equation*}
    By Assumption \ref{assume:CLT}, we have $\E{\abs{ f_{t,lh} }^m} \le C < \infty$ for any $l\in [k]$ and $h\in[r]$. Similarly, we have $\E{\abs{x_{t}}^m} \le C$.
    Then Theorem 2.20 in \cite{fan2008nonlinear} implies the desired result.

    Next, we have, using convexity of $\norm{\cdot}^2$,
    \begin{equation*}
        \begin{aligned}
            \E{\norm{\sqrt{\frac{T}{q}} \sum_{j=1}^{q}\bar e_{ij}\bar\bF}^2}
            & = \E{\norm{ \frac{1}{T \sqrt{qT}} \sum_{j=1}^{q}  \sum_{t=1}^T \sum_{s=1}^{T} e_{t,ij} \bF_s }^2}
            \le \E{  \frac{1}{T} \sum_{s=1}^{T} \norm{ \frac{1}{\sqrt{qT}} \sum_{j=1}^{q}  \sum_{t=1}^T e_{t,ij}}^2 \norm{ \bF_s }^2} \\
            & = \bigO{1}.
        \end{aligned}
    \end{equation*}


    \underline{\sc Step 2.} Now we show results in Lemma \ref{assume:factor_noise_weak_corr_0}.
    Plugging in $\tilde e_{t, ij} \defeq e_{t, ij} + \tilde\alpha \bar e_{ij}$, $\tilde \bF_t \defeq \bF_t + \tilde\alpha \bar\bF$ and using the fact that $2\tilde\alpha + \tilde\alpha^2 = \alpha$,  we have
    \begin{eqnarray}
        \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \tilde e_{t, ij} \tilde \bF_{t} & = & \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, ij}\bF_{t} + \tilde\alpha \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t,ij} \bar\bF \nonumber \\
        &  & + \tilde\alpha \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \bar e_{ij} \bF_{t} + \tilde\alpha^2 \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \bar e_{ij} \bar\bF \nonumber \\
        & = & \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, ij}\bF_{t} + \alpha \sqrt{\frac{T}{q}} \sum_{j=1}^{q}\bar e_{ij}\bar\bF \nonumber
    \end{eqnarray}

    Thus equation \eqref{eqn:lemma-fn-1} implies $\E{\norm{\frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \tilde e_{t, ij} \tilde \bF_{t}}^2} = \bigO{1}$.
    Similarly, equation \eqref{eqn:lemma-fn-2} implies $\E{ \norm{\frac{1}{\sqrt{p T}} \sum_{t=1}^{T} \sum_{i=1}^{p} \tilde e_{t, ij} \tilde \bF_{t}}^2} = \bigO{1}$.

\end{proof}


\begin{lemma} \label{assume:ef}
Under Assumption \ref{assume:alpha-mixing} - \ref{assume:CLT}, we have,
\begin{enumerate}[label=(\alph*) ]
\item For any $l\in [p]$, $\norm{ \frac{1}{ \sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, lj} \bC_{j \cdot}^\top \bF_t^\top }^2 = \Op{1}$.
\item $\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \bR^\top \bE_t \bC \bF_t^\top = \Op{1}$.
\item For any $i, l \in [p]$ and $j, h \in [q]$, $\abs{ \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \left( e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} \right) } = \Op{1}$.
\item For any row $i\in [p]$, $\abs{ \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \paran{ e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} } }= \Op{1}$.
\end{enumerate}
\end{lemma}
\begin{proof}
\begin{enumerate}[label=(\alph*) ]
\item By Lemma Assumption \ref{assume:factor_noise_weak_corr_0}, we have $\norm{ \frac{1}{ \sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \paran{e_{t, lj} \bF_t^\top - \E{e_{t, lj} \bF_t^\top}} } = \Op{1}$.
\begin{equation*}
\begin{aligned}
\norm{ \frac{1}{ \sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, lj} \bC_{j \cdot}^\top \bF_t^\top }^2
& \le \norm{ \frac{2}{ \sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \paran{e_{t, lj} \bC_{j \cdot}^\top \bF_t^\top - \E{e_{t, lj} \bC_{j \cdot}^\top \bF_t^\top}} }^2
+ \norm{ \E{ \frac{2}{ \sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, lj} \bC_{j \cdot}^\top \bF_t^\top} }^2 \\
& \le \max_{j\in[q]}\norm{\bC_{j \cdot}}^2 \cdot \norm{ \frac{1}{ \sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \paran{e_{t, lj} \bF_t^\top - \E{e_{t, lj} \bF_t^\top}} }^2  \\
& + \max_{j\in[q]}\norm{\bC_{j \cdot}}^2 \cdot \E{ \norm{ \frac{1}{ \sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q}  \bF_t^\top e_{t, lj} }^2 } \qquad \text{by Jensen's Inequality}
% & = \Op{1}.
\end{aligned}
\end{equation*}
By Assumption \ref{assume:factor_noise_weak_corr_0} (c), we have $\E{e_{t, lj} \bF_t^\top} = \bzero$.
By Lemma \ref{assume:factor_noise_weak_corr_0} and Markov inequality, we have $\frac{1}{ \sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \paran{e_{t, lj} \bF_t^\top - \E{e_{t, lj} \bF_t^\top}} = \Op{1}$.
Since $\bC_{j \cdot} \in \RR^r$, we also have $\max_j \norm{ \bC_{j \cdot} }^2 = \bigO{1}$.
Together with Lemma \ref{assume:factor_noise_weak_corr_0} and the fact that $\bF_t$ are of fixed dimensions, we obtain the final result.

\item Note that the matrix in consideration is of finite dimension and bounded second moment. The final result follows from Lemma \ref{assume:moments_0} and Markov inequality.

\item Follow from Lemma \ref{assume:moments_Et_0} and Markov inequality.

\item Follow from Lemma \ref{assume:moments_0} and Markov inequality.

\end{enumerate}
\end{proof}

%Under Assumptions \ref{assume:alpha-mixing}, \ref{assume:factor-noise-matrix} and \ref{assume:loading_matrix}, an application of Proposition 2.8 and Theorem 2.20 in \cite{fan2008nonlinear} implies that, as $T \rightarrow \infty$, we have $\frac{1}{T} \sum_{t=1}^{T} \bF_t \convprob \bmu_F$,
%\[
%\frac{1}{qT}\sum_{t=1}^T\paran{\bF_t-\bar\bF}\bC^\top\bC\paran{\bF_t-\bar\bF}^\top \convprob \bSigma_{FC} \quad\text{and}\quad \frac{1}{pT}\sum_{t=1}^T\paran{\bF_t-\bar\bF}^\top\bR^\top\bR\paran{\bF_t-\bar\bF} \convprob \bSigma_{FR}.
%\]
%for some positive definite matrices $\bSigma_{FC}$ of dimension $k \times k$ and $\bSigma_{FR}$ of dimension $r \times r$.
%Let $\tilde\alpha=\sqrt{\alpha+1}-1$ and $\tilde\bF \defeq \bF_t+\tilde\alpha\bar\bF$.
%Similarly, we have that, using $2\tilde\alpha+\tilde\alpha^2=\alpha$,
%\begin{equation*}
%    \frac{1}{qT}\sum_{t=1}^T\tilde\bF_t \bC^\top\bC \tilde\bF_t^\top \convprob \tilde\bSigma_{FC} , \quad\text{and}\quad \frac{1}{pT}\sum_{t=1}^T\tilde\bF_t^\top\bR^\top\bR\tilde\bF_t \convprob \tilde\bSigma_{FR}.
%\end{equation*}
%where $\tilde\bSigma_{FC} = \bSigma_{FC} + \paran{1+\alpha} \bmu_F (\bC^\top\bC/q) \bmu_F^\top$ and $\tilde\bSigma_{FR} = \bSigma_{FR} + \paran{1+\alpha} \bmu_F (\bR^\top\bR/p) \bmu_F^\top$.

==> miscs <==


\begin{assumption}\label{assume:factor_noise_weak_corr}
\textbf{Weak dependence between factor $\bF_t$ and noise $\bE_t$.}
For any $1 \le i \le p$, there exists a positive constant $C < \infty$ such that for all $p$, $q$ and $T$,
\begin{enumerate}
\item $\E{\norm{\frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, ij}\bF_{t}}^2}\le C$ and
$\E{\norm{\sqrt{\frac{T}{q}} \sum_{j=1}^{q}\bar e_{ij}\bar\bF}^2} \le C$.
\item $\E{\norm{\frac{1}{\sqrt{p T}} \sum_{t=1}^{T} \sum_{i=1}^{p} e_{t, ij}\bF_{t}}^2}\le C$ and $\E{\norm{\sqrt{\frac{T}{p}} \sum_{i=1}^{p}\bar e_{ij}\bar\bF}^2} \le C$.
\end{enumerate}
\end{assumption}

\begin{assumption} \label{assume:moments_CLT}
\textbf{Moments condition.}  There exists a positive $C<\infty$ such that for all $p$, $q$ and $T$,
\begin{enumerate}[label=(\alph*)]

\item For any row $i\in[p]$,
\[
\mathbb{E} \norm{ \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \bR_{l \cdot} \left( e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} \right)}^2  \le C,
\quad
\mathbb{E} \norm{\sqrt{\frac{T}{p q}} \sum_{l=1}^{p} \sum_{j=1}^{q} \bR_{l \cdot} \paran{ \bar e_{lj} \bar e_{ij} - \E{\bar e_{lj} \bar e_{ij}} }} ^2  \le C.
\]
Similarly, for any column $j\in[q]$,
\[
\mathbb{E} \norm{ \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{i=1}^{p} \sum_{h=1}^{q} \bC_{h \cdot} \left( e_{t, ih} e_{t, ij} - \E{e_{t, ih} e_{t, ij}} \right)}^2  \le C,
\quad
\mathbb{E} \norm{\sqrt{\frac{T}{p q}} \sum_{i=1}^{p} \sum_{h=1}^{q} \bC_{h \cdot} \paran{\bar e_{ih} \bar e_{ij} - \E{\bar e_{ih} \bar e_{ij}} } } ^2  \le C.
\]

\item The $k \times k$ matrix satisfies
\[
\mathbb{E}\,\norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \bR^\top \bE_t \bC \bF_t^\top}^2_2\le C, \quad\text{and}\quad \mathbb{E}\,\norm{\frac{\sqrt{T}}{\sqrt{pq}} \bR^\top \bar\bE\bC\bar\bF^\top}\le C.
\]
Similarly, the $r \times r$ matrix satisfies
\[
\mathbb{E} \, \norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \bF_t^\top \bR^\top \bE_t \bC }^2_2\le C, \quad\text{and}\quad \mathbb{E}\,\norm{\frac{\sqrt{T}}{\sqrt{pq}} \bar\bF^\top\bR^\top \bar\bE\bC}\le C.
\]

\item For each row $i$, as $q, T \rightarrow \infty$,
\[
\begin{pmatrix}
\frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \bF_t \bC^\top \be_{t, i \cdot} \\
\frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \bC^\top \be_{t, i \cdot}
\end{pmatrix} \convdist \calN \paran{\bzero, \begin{pmatrix}
\bPhi_{R, i, 11} & \bPhi_{R, i, 12} \\
\bPhi_{R, i, 21} & \bPhi_{R, i, 22}
\end{pmatrix}},
\]
where
\begin{equation*}
\begin{aligned}
\bPhi_{R, i, 11} & = \underset{q, T \rightarrow \infty}{{\rm p lim}} \frac{1}{qT}  \sum_{t=1}^{T} \sum_{s=1}^{T} \bF_t \bC^\top \be_{t, i \cdot} \be_{s, i \cdot}^\top \bC \bF_s^\top, \\
\bPhi_{R, i, 12} & = \bPhi_{R, i, 21}^\top = \underset{q, T \rightarrow \infty}{{\rm p lim}} \frac{1}{qT}  \sum_{t=1}^{T} \sum_{s=1}^{T} \bF_t \bC^\top \be_{t, i \cdot} \be_{s, i \cdot}^\top \bC, \\
\bPhi_{R, i, 22} & = \underset{q, T \rightarrow \infty}{{\rm p lim}} \frac{1}{qT}  \sum_{t=1}^{T} \sum_{s=1}^{T} \bC^\top \be_{t, i \cdot} \be_{s, i \cdot}^\top \bC.
\end{aligned}
\end{equation*}
\item For each column $j$, as $p, T \rightarrow \infty$,
\[
\begin{pmatrix}
\frac{1}{\sqrt{pT}} \sum_{t=1}^{T} \bF_t^\top \bR^\top \be_{t, \cdot j }  \\
\frac{1}{\sqrt{pT}} \sum_{t=1}^{T} \bR^\top \be_{t, \cdot j}
\end{pmatrix} \convdist \calN \paran{ \bzero, \begin{pmatrix}
\bPhi_{C, j, 11} & \bPhi_{C, j, 12} \\
\bPhi_{C, j, 21} & \bPhi_{C, j, 22}
\end{pmatrix} },
\]
where
\begin{equation*}
\begin{aligned}
\bPhi_{C,j,11} & = \underset{q, T \rightarrow \infty}{{\rm p lim}} \frac{1}{pT} \sum_{t=1}^{T} \sum_{s=1}^{T} \bF_t^\top \bR^\top \be_{t, \cdot j} \be_{s, \cdot j}^\top \bR \bF_s, \\
\bPhi_{C,j,12} & = \bPhi_{C,j,21}^\top = \underset{q, T \rightarrow \infty}{{\rm p lim}} \frac{1}{qT}  \sum_{t=1}^{T} \sum_{s=1}^{T} \bF_t^\top \bR^\top \be_{t, \cdot j} \be_{s, \cdot j}^\top \bR, \\
\bPhi_{C,j,22} & = \underset{q, T \rightarrow \infty}{{\rm p lim}} \frac{1}{qT}  \sum_{t=1}^{T} \sum_{s=1}^{T} \bR^\top \be_{t, \cdot j} \be_{s, \cdot j}^\top \bR.
\end{aligned}
\end{equation*}
\end{enumerate}
\end{assumption}


==> proofs-B.tex <==
%!TEX root = 0-main.tex


\section{Proofs of Lemma \ref{assume:factor_matrix_0} - \ref{assume:CLT_0}} \label{sec:proof-B}

%Recall that $\YY_R \defeq \brackets{\bY_1 \; \cdots \; \bY_T} \in \RR^{p \times qT}$, $\YY_C \defeq \brackets{\bY_1^\top \; \cdots \; \bY_T^\top} \in \RR^{q \times pT}$, $\tilde \YY_R = \YY_R \paran{\bW \otimes \bI_p}$ and $\tilde \YY_C = \YY_C \paran{\bW \otimes \bI_q}$ where $\bW = \bI_T + \tilde \alpha \cdot \frac{\bbone_T \bbone_T^\top}{T}$ with $\tilde \alpha = \sqrt{\alpha +1} - 1$ and $\bW^2 = \bI_T + \alpha \cdot \frac{\bbone_T \bbone_T^\top}{T}$.


%\subsection{Proofs of Lemma 2 - 8} \label{sec:cond'n-A-E}

We prove Lemma \ref{assume:factor_matrix_0} - \ref{assume:CLT_0} under Assumption \ref{assume:alpha-mixing} - \ref{assume:CLT}.
In the following proofs, we repeated use the fact that $\tilde e_{t, ij} \defeq e_{t, ij} + \tilde\alpha \bar e_{ij}$, $\tilde \bF_t \defeq \bF_t + \tilde\alpha \bar\bF$ and $2\tilde\alpha + \tilde\alpha^2 = \alpha$.



\paragraph{Proof of Lemma \ref{assume:factor_matrix_0}.}

\begin{proof}
    Under Assumptions \ref{assume:alpha-mixing}, \ref{assume:factor-noise-matrix} and \ref{assume:loading_matrix}, an application of Proposition 2.8 and Theorem 2.20 in \cite{fan2008nonlinear} implies that, as $T \rightarrow \infty$, we have $\frac{1}{T} \sum_{t=1}^{T} \bF_t \convprob \bmu_F$,
    \[
    \frac{1}{qT}\sum_{t=1}^T\paran{\bF_t-\bar\bF}\bC^\top\bC\paran{\bF_t-\bar\bF}^\top \convprob \bSigma_{FC} \quad\text{and}\quad \frac{1}{pT}\sum_{t=1}^T\paran{\bF_t-\bar\bF}^\top\bR^\top\bR\paran{\bF_t-\bar\bF} \convprob \bSigma_{FR},
    \]
    where $\bSigma_{FC}$ and $\bSigma_{FR}$ are defined in \eqref{eqn:Sigma_FC_FR}.
    Plugging in $\tilde\bF \defeq \bF_t+\tilde\alpha\bar\bF$ and using the fact that $\tilde\alpha=\sqrt{\alpha+1}-1$, $2\tilde\alpha+\tilde\alpha^2=\alpha$, we have that,
    \begin{equation*}
        \frac{1}{qT}\sum_{t=1}^T\tilde\bF_t \bC^\top\bC \tilde\bF_t^\top \convprob \tilde\bSigma_{FC} , \quad\text{and}\quad \frac{1}{pT}\sum_{t=1}^T\tilde\bF_t^\top\bR^\top\bR\tilde\bF_t \convprob \tilde\bSigma_{FR}.
    \end{equation*}
    where $\tilde\bSigma_{FC} = \bSigma_{FC} + \paran{1+\alpha} \bmu_F (\bC^\top\bC/q) \bmu_F^\top$ and $\tilde\bSigma_{FR} = \bSigma_{FR} + \paran{1+\alpha} \bmu_F (\bR^\top\bR/p) \bmu_F^\top$.


        we have $\E{\norm{\tilde\bF_t}^4} \le c \E{\norm{\bF_t}^4} \le C < \infty$.

        Using $2\tilde\alpha+\tilde\alpha^2=\alpha$, we have
        \begin{equation*}
            \frac{1}{qT}\sum_{t=1}^T\tilde\bF_t \bC^\top\bC \tilde\bF_t^\top \convprob \tilde\bSigma_{FC} , \quad\text{and}\quad \frac{1}{pT}\sum_{t=1}^T\tilde\bF_t^\top\bR^\top\bR\tilde\bF_t \convprob \tilde\bSigma_{FR}.
        \end{equation*}
        where $\tilde\bSigma_{FC} = \bSigma_{FC} + \paran{1+\alpha} \bmu_F (\bC^\top\bC/q) \bmu_F^\top$ and $\tilde\bSigma_{FR} = \bSigma_{FR} + \paran{1+\alpha} \bmu_F (\bR^\top\bR/p) \bmu_F^\top$ are positive definite.
\end{proof}



\paragraph{Proof of Lemma \ref{assume:cross_row_col_corr_0}.}
\begin{proof}~
Plugging $\tilde\bE_t = \bE_t + \tilde\alpha\bar\bE$ in the definition that $ \tilde\bU_E \;\defeq\; \E{\frac{1}{qT} \sum_{t=1}^{T} \tilde\bE_t\tilde\bE_t^\top}$
and using the fact that $\tilde\alpha \defeq \sqrt{\alpha + 1} - 1$, we derive
\begin{enumerate}[label=(\alph*)]
    \item $\E{\tilde e_{t, ij}} = 0$ and $\EE \lvert \tilde e_{t, ij} \rvert^8 = \bigO{1}$.
    \item  We have
    \[
    \tilde\bU_E =  \bU_E + \E{\frac{\alpha}{q} \bar\bE \bar\bE^\top} \le \paran{1+\alpha}\bU_E.
    \]
    Similarly for $\tilde\bV_E$, we have
    \[
    \tilde\bV_E =  \bV_E + \E{\frac{\alpha}{q} \bar\bE^\top \bar\bE} \le \paran{1+\alpha}\bV_E.
    \]
    The results follow from Assumption \ref{assume:cross_row_col_corr}.
\end{enumerate}
\begin{comment}
     \begin{enumerate}[label=\ref{cond:cross_row_col_corr}.\arabic*]
         \setcounter{enumi}{1}
         \item By definition,
         $$\bU_E = \E{\frac{1}{qT} \sum_{t=1}^{T}\bE_t \bE_t^T} = \E{\frac{1}{qT} \sum_{t=1}^{T} \sum_{j=1}^{q} \be_{t,\cdot j} \be_{t, \cdot j}^T} = \frac{1}{qT} \sum_{t=1}^{T} \sum_{j=1}^{q}  \brackets{\Cov{e_{t, lj} e_{t, kj}}}_{1\le l, k \le p}.$$
          By Davydov's inequality (Corollary 16.2.4 in \cite{athreya2006measure}), there is a constant $C>0$, for all $i,j \in [q]$, and $s, t \in [T]$, $\abs{ \Cov{e_{t, lj}, e_{t, kj} } } = \bigO{1} \alpha( \abs{l-k} )^{1 - 2/\gamma}$.
         Under $\alpha$-mixing over rows in Assumption \ref{assume:cross_row_col_corr}, we have $\sum_{ h > 1 } \alpha( h )^{1 - 2/\gamma} \le \infty$.
         Thus, $\norm{ \bU_E }_1 = \bigO{1}$.
         Similarly, we have $\norm{ \bV_E }_1 = \bigO{1}$.

%         \item Under Assumptions \ref{assume:factor-noise-matrix} and \ref{assume:cross_row_col_corr}, an application of Proposition 2.8 and Theorem 2.20 in \cite{fan2008nonlinear} implies that
%         \begin{equation*}
%             \begin{aligned}
%                 \bU_E & = \E{\frac{1}{qT} \sum_{t=1}^{T}\bE_t \bE_t^T} = \E{\frac{1}{qT} \sum_{t=1}^{T} \sum_{j=1}^{q} \be_{t,\cdot j} \be_{t, \cdot j}^T} \\
%                 & =
%             \end{aligned}
%         \end{equation*}
     \end{enumerate}
\end{comment}
\end{proof}

\paragraph{Proof of Lemma \ref{assume:temporal_dependence_0}.}

\begin{proof}
\underline{\sc Step 1.} We first show that
\begin{equation} \label{eqn:lemma-td-1}
    \sum_{s=1}^{T} \norm{ \E{ \frac{1}{p q} \bR^\top \bE_s \bE_t^\top \bR } }= \bigO{1}
    \quad\text{and}\quad
    \sum_{s=1}^{T} \norm{ \E{ \frac{1}{p q} \bC^\top \bE_s^\top \bE_t \bC} }= \bigO{1}.
    \end{equation}

By Davydov's inequality (Corollary 16.2.4 in \cite{athreya2006measure}), there is a constant $C>0$, for any $i,l \in [p]$, $j\in [q]$, and $s, t \in [T]$, $\abs{ \E{e_{s,ij}e_{t,lj}} } \le c \cdot \alpha( \abs{t-s} )^{1 - 2/\gamma}$.
Under $\alpha$-mixing Assumption \ref{assume:alpha-mixing}, we have $\sum_{ h > 1 } \alpha( h )^{1 - 2/\gamma} = \bigO{1}$.
\begin{equation*}
    \begin{aligned}
    \sum_{s=1}^{T} \norm{ \E{ \frac{1}{p q} \bR^\top \bE_s \bE_t^\top \bR } }
    & \le \sum_{s=1}^{T} \norm{\frac{1}{q} \sum_{j=1}^q \E{\be_{s,\cdot j} \be_{t,\cdot j}^\top } }\cdot \norm{\bR}^2 / p
    = \bigO{1}.
    \end{aligned}
\end{equation*}
The second equation in \eqref{eqn:lemma-td-1} follows by a similar argument.

\underline{\sc Step 2.} Now we show results in Lemma \ref{assume:temporal_dependence_0}.
Plugging in $\tilde\bE_t \defeq \bE_t + \tilde\alpha\bar\bE$ and using the fact that $2\tilde\alpha + \tilde\alpha^2 = \alpha$, we have
\begin{equation*}
    \begin{aligned}
    \sum_{s=1}^{T} \norm{ \E{ \frac{1}{p q} \bR^\top \tilde\bE_s \tilde\bE_t^\top \bR } }
    & \le  \sum_{s=1}^{T} \norm{ \E{ \frac{1}{p q} \bR^\top \bE_s \bE_t^\top \bR } }
     + \; \tilde \alpha \sum_{s=1}^{T} \frac{1}{T} \sum_{t=1}^{T} \norm{ \E{ \frac{1}{p q} \bR^\top \bE_s \bE_t^\top \bR } } \\
    &  + \; \tilde \alpha \sum_{s=1}^{T} \frac{1}{T} \sum_{s=1}^{T} \norm{ \E{ \frac{1}{p q} \bR^\top \bE_s \bE_t^\top \bR } }
    + \; \tilde \alpha^2 \sum_{s=1}^{T} \frac{1}{T^2} \sum_{s=1}^{T} \sum_{t=1}^{T} \norm{ \E{ \frac{1}{p q} \bR^\top \bE_s \bE_t^\top \bR } } \nonumber \\
    & \le \paran{1 + \alpha} \sum_{s=1}^{T} \norm{ \E{ \frac{1}{p q} \bR^\top \bE_s \bE_t^\top \bR } }\nonumber \\
    & = \bigO{1}.
   \end{aligned}
\end{equation*}
By similar argument, we obtain $\sum_{s=1}^{T} \norm{ \E{ \frac{1}{p q} \bC^\top \tilde\bE_s^\top \tilde\bE_t \bC} } = \bigO{1}$.

\end{proof}


\paragraph{Proof of Lemma \ref{assume:factor_noise_weak_corr_0}.}

\begin{proof}

\underline{\sc Step 1.} We first show that
for any $i \in [p]$,  $j\in[q]$,
\begin{eqnarray}
&\E{\norm{\frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, ij}\bF_{t} \bC_{j\cdot}}^2} = \bigO{1}, \quad
\E{\norm{\sqrt{\frac{T}{q}} \sum_{j=1}^{q}\bar e_{ij}\bar\bF \bC_{j\cdot}}^2} = \bigO{1}, \label{eqn:lemma-fn-1} \\
&\E{\norm{\frac{1}{\sqrt{p T}} \sum_{t=1}^{T} \sum_{i=1}^{p} e_{t, ij}\bF_{t}^\top \bR_{i\cdot}}^2} = \bigO{1}, \quad
\E{\norm{\sqrt{\frac{T}{p}} \sum_{i=1}^{p}\bar e_{ij}\bar\bF^\top \bR_{i\cdot}}^2} = \bigO{1}. \label{eqn:lemma-fn-2}
\end{eqnarray}

Proofs for \eqref{eqn:lemma-fn-1} and \eqref{eqn:lemma-fn-2} are the same. Here we only present the proof for \eqref{eqn:lemma-fn-1}.

For any $i\in[p]$ and $t\in [T]$, we define a random vector $\bx_t = \frac{1}{\sqrt{q}} \sum_{j=1}^q \bC_{j\cdot} e_{t, i j}$, which is $\alpha$-mixing over $t$.
We rewrite $ \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, ij}\bF_{t} \bC_{j\cdot} = \frac{1}{\sqrt{T}} \sum_{t=1}^{T} \bF_t\bx_t$.
By Assumption \ref{assume:factor-noise-matrix}, we have $\E{\bF_t\bx_t} = 0$.

Now we show that there exists some $m > 2$ such that $\EE\norm{\bF_t \bx_t}^m \le C <\infty$.
Since $\bF_t$ is of fixed dimensions, it suffices to show that $\E{\paran{\bff_{t,l\cdot}^\top\bx_t}^m} \le C$ and $\E{x_{t,h}^m} \le C$ for any $l\in [k]$ and $h \in [r]$.

By Holder inequality, we have for any $1< a, b < \infty$ and $1/a + 1/b = 1$,
\begin{equation*}
    \E{\paran{\bff_{t,l\cdot}^\top\bx_t}^m}
    \le \E{\norm{\bff_{t,l\cdot}}^m \norm{\bx_t}^m}
    \le \paran{ \E{\norm{\bff_{t,l\cdot}}^{ma} } }^{1/a} \paran{\E{\norm{\bx_t}^{mb}}}^{1/b}.
\end{equation*}
By Assumption \ref{assume:CLT}, we have $\E{\paran{\bff_{t,l\cdot}^\top\bx_t}^m} \le C$ for any $l\in [k]$. Similarly, we have $\E{x_{t,h}^m} \le C$ for any $h \in [r]$.
Then Theorem 2.20 in \cite{fan2008nonlinear} implies the desired result.

Next, we have, using convexity of $\norm{\cdot}^2$,
\begin{equation*}
    \begin{aligned}
        \E{\norm{\sqrt{\frac{T}{q}} \sum_{j=1}^{q}\bar e_{ij}\bar\bF \bC_{j\cdot}}^2}
        & = \E{\norm{ \frac{1}{T \sqrt{qT}} \sum_{j=1}^{q}  \sum_{t=1}^T \sum_{s=1}^{T} e_{t,ij} \bF_s \bC_{j\cdot} }^2}
        \le \E{  \frac{1}{T} \sum_{s=1}^{T} \norm{ \frac{1}{\sqrt{qT}} \sum_{j=1}^{q}  \sum_{t=1}^T e_{t,ij}\bC_{j\cdot} }^2 \norm{ \bF_s }^2} \\
        & = \bigO{1}.
    \end{aligned}
\end{equation*}


\underline{\sc Step 2.} Now we show results in Lemma \ref{assume:factor_noise_weak_corr_0}.
Plugging in $\tilde e_{t, ij} \defeq e_{t, ij} + \tilde\alpha \bar e_{ij}$, $\tilde \bF_t \defeq \bF_t + \tilde\alpha \bar\bF$ and using the fact that $2\tilde\alpha + \tilde\alpha^2 = \alpha$,  we have
\begin{eqnarray}
\frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \tilde e_{t, ij} \tilde \bF_{t} \bC_{j\cdot} & = & \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, ij}\bF_{t} \bC_{j\cdot} + \tilde\alpha \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t,ij} \bar\bF \bC_{j\cdot} \nonumber \\
&  & + \tilde\alpha \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \bar e_{ij} \bF_{t} \bC_{j\cdot} + \tilde\alpha^2 \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \bar e_{ij} \bar\bF \bC_{j\cdot} \nonumber \\
& = & \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, ij}\bF_{t}\bC_{j\cdot} + \alpha \sqrt{\frac{T}{q}} \sum_{j=1}^{q}\bar e_{ij}\bar\bF\bC_{j\cdot} \nonumber
\end{eqnarray}

Thus equation \eqref{eqn:lemma-fn-1} implies $\E{\norm{\frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \tilde e_{t, ij} \tilde \bF_{t} \bC_{j\cdot}}^2} = \bigO{1}$.
Similarly, equation \eqref{eqn:lemma-fn-2} implies $\E{ \norm{\frac{1}{\sqrt{p T}} \sum_{t=1}^{T} \sum_{i=1}^{p} \tilde e_{t, ij} \tilde \bF_{t} \bC_{j\cdot}}^2} = \bigO{1}$.

\end{proof}



\paragraph{Proof of Lemma \ref{assume:moments_0}.}
\begin{proof}
\begin{enumerate}[label=(\alph*)]
    \item
    \underline{\sc Step 1.} We firstly prove \eqref{eqn:mom-0-1} and \eqref{eqn:mom-0-2} stated as follows..
    For any row $i\in[p]$,
    \begin{equation} \label{eqn:mom-0-1}
    \mathbb{E} \paran{ \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} \right)}^2  = \bigO{1},
    \quad
    \mathbb{E} \paran{\sqrt{\frac{T}{p q}} \sum_{l=1}^{p} \sum_{j=1}^{q} \paran{ \bar e_{lj} \bar e_{ij} - \E{\bar e_{lj} \bar e_{ij}} }} ^2  = \bigO{1}.
    \end{equation}
    Similarly, for any column $j\in[q]$,
    \begin{equation} \label{eqn:mom-0-2}
    \mathbb{E} \paran{ \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{i=1}^{p} \sum_{h=1}^{q} \left( e_{t, ih} e_{t, ij} - \E{e_{t, ih} e_{t, ij}} \right)}^2  = \bigO{1},
    \quad
    \mathbb{E} \paran{\sqrt{\frac{T}{p q}} \sum_{i=1}^{p} \sum_{h=1}^{q} \paran{\bar e_{ih} \bar e_{ij} - \E{\bar e_{ih} \bar e_{ij}} } } ^2  = \bigO{1}.
    \end{equation}

    For equation \eqref{eqn:mom-0-1}, we have that, under Assumption \ref{assume:cross_row_col_corr} (b), for any row $i$,
    \begin{equation*}
     \begin{aligned}
         & \mathbb{E} \paran{ \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} \right)}^2 \\
         & = \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \abs{ \Cov{e_{t, lj} e_{t, ij}, \; e_{t, lj} e_{t, ij} } }
         + \frac{1}{p q T}
             \sum_{t=1}^{T}
             \sum_{l=1}^{p}
             \sum_{j=1}^{q}
             \paran{
             \sum_{s=1}^T
             \sum_{m=1}^p
             \sum_{ \substack{h \in [q] \\ h\ne [j]}  }
             \abs{ \Cov{ e_{t, lj} e_{t, ij}, \;e_{s, mh} e_{s, ih} } } } \\
         & = \bigO{1}.
     \end{aligned}
    \end{equation*}
    Then,
    \begin{equation*}
     \begin{aligned}
         \mathbb{E} \paran{\sqrt{\frac{T}{p q}} \sum_{l=1}^{p} \sum_{j=1}^{q} \paran{ \bar e_{lj} \bar e_{ij} - \E{\bar e_{lj} \bar e_{ij}} }} ^2
         & =  \mathbb{E} \paran{ \frac{1}{T} \sum_{s=1}^T \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( e_{s, lj} e_{t, ij} - \E{e_{s, lj} e_{t, ij}} \right)}^2 \\
         & \le  \frac{1}{T} \sum_{s=1}^T \mathbb{E} \paran{ \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( e_{s, lj} e_{t, ij} - \E{e_{s, lj} e_{t, ij}} \right)}^2 \\
         & = \bigO{1}.
     \end{aligned}
    \end{equation*}
    The proofs of \eqref{eqn:mom-0-2} for any column $j$ are similar.

    \underline{\sc Step 2.} Now we show the final results of Lemma \ref{assume:moments_0} (a).
    We have, for all row $i$,
    \begin{eqnarray*}
        & &\norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T}\sum_{l=1}^{p}\sum_{j=1}^{q} \paran{ \tilde e_{t, lj} \tilde e_{t, ij} - \E{\tilde e_{t, lj} \tilde e_{t, ij}} }} \\
        &\le & \norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \paran{e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} }} + \norm{\frac{\tilde\alpha}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \paran{ e_{t, lj} \bar e_{ij} - \E{e_{t, lj} \bar e_{ij}} }} \\
        & + &\;\norm{\frac{\tilde\alpha}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \paran{\bar e_{lj} e_{t, ij} - \E{\bar e_{lj} e_{t, ij}} }} + \;\norm{\frac{\tilde\alpha^2}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \paran{\bar e_{lj} \bar e_{ij} - \E{\bar e_{lj} \bar e_{ij}} }}.\\
        & = & \norm{\frac{1}{\sqrt{pqT}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \paran{e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} }} + 2\alpha\norm{\sqrt{\frac{T}{p q}} \sum_{l=1}^{p} \sum_{j=1}^{q} \bR_{l \cdot} \paran{ \bar e_{lj} \bar e_{ij} - \E{\bar e_{lj} \bar e_{ij}} }}.
    \end{eqnarray*}
    Equation \eqref{eqn:mom-0-2} therefore implies
    \[
    \mathbb{E} \norm{ \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( \tilde e_{t, lj} \tilde e_{t, ij} - \E{\tilde e_{t, lj} \tilde e_{t, ij}} \right)}^2 = \bigO{1}.
    \]
    The remaining part for the columns can be derived in the same way.

    \item
    \underline{\sc Step 1.} We firstly prove \eqref{eqn:lemma-mom-0-3} and \eqref{eqn:lemma-mom-0-4} stated as follows.
    The $k \times k$ matrix satisfies
    \begin{equation} \label{eqn:lemma-mom-0-3}
    \mathbb{E}\,\norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \bR^\top \bE_t \bC \bF_t^\top}^2_2= \bigO{1}, \quad\text{and}\quad \mathbb{E}\,\norm{\frac{\sqrt{T}}{\sqrt{pq}} \bR^\top \bar\bE\bC\bar\bF^\top}= \bigO{1}.
    \end{equation}
    Similarly, the $r \times r$ matrix satisfies
    \begin{equation} \label{eqn:lemma-mom-0-4}
    \mathbb{E} \, \norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \bF_t^\top \bR^\top \bE_t \bC }^2_2= \bigO{1}, \quad\text{and}\quad \mathbb{E}\,\norm{\frac{\sqrt{T}}{\sqrt{pq}} \bar\bF^\top\bR^\top \bar\bE\bC}= \bigO{1}.
    \end{equation}
    For \eqref{eqn:lemma-mom-0-3}, we have
    \begin{equation*}
        \begin{aligned}
             \mathbb{E}\,\norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \bR^\top \bE_t \bC \bF_t^\top}^2
             & =  \mathbb{E}\,\norm{ \frac{1}{\sqrt{T}} \sum_{t=1}^{T} \paran{ \frac{1}{\sqrt{p q}} \sum_{i=1}^p \sum_{j=1}^q \bR_{i \cdot} \bC_{j \cdot}^\top  e_{t,ij} } \bF_t^\top}^2.
        \end{aligned}
    \end{equation*}
    The rest of the proof of  is similar to that of \eqref{eqn:lemma-fn-1} by setting $\bX_t = \frac{1}{\sqrt{pq}} \sum_{i=1}^p \sum_{j=1}^q \bR_{i \cdot} \bC_{j \cdot}^\top e_{t, i j}$ and using Assumption \ref{assume:CLT}, and Theorem 2.20 in \cite{fan2008nonlinear}.

    \underline{\sc Step 2.} Now we show the final results of Lemma \ref{assume:moments_0} (b).
    We have
    \begin{eqnarray*}
        \norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \bR^\top \tilde\bE_t \bC \tilde\bF_t^\top} & \le \norm{\frac{1}{\sqrt{p q T}}\sum_{t=1}^{T} \bR^\top\bE_t\bC\bF_t^\top} + 2\alpha\norm{\frac{\sqrt{T}}{\sqrt{pq}} \bR^\top \bar\bE\bC\bar\bF^\top}
    \end{eqnarray*}

    Equation \eqref{eqn:lemma-mom-0-3} therefore implies that the $k \times k$ matrix satisfies
    \[
    \mathbb{E} \, \norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \bR^\top \tilde\bE_t \bC \tilde\bF_t^\top}^2_2 = \bigO{1}
    \]
    Similarly, from equation \eqref{eqn:lemma-mom-0-4}, the $r \times r$ matrix satisfies
    \[
    \mathbb{E} \, \norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \tilde\bF_t^\top\bR^\top\tilde\bE_t\bC }^2_2 = \bigO{1}
    \]
\end{enumerate}
\end{proof}


\paragraph{Proof of Lemma \ref{assume:moments_Et_0}}

\begin{proof} ~
     \begin{enumerate}[label=(\alph*)]
        \setcounter{enumi}{0}
        \item
        \underline{\sc Step 1.} We firstly prove \eqref{eqn:lemma-mE-1} stated as follows.
        For any $i,l \in [p]$ and $j,h \in [q]$,
        \begin{equation} \label{eqn:lemma-mE-1}
            \begin{aligned}
                & \EE\abs{ \frac{1}{qT} \sum_{t=1 }^{T} \sum_{j=1}^{q} \paran{e_{t, ij} e_{t, lj} - \E{ e_{t, ij} e_{t, lj} }} }^2 = \bigO{\frac{1}{qT}},
                & \EE\abs{ \frac{1}{q} \sum_{j=1}^{q} \paran{\bar e_{ij} \bar e_{lj} - \E{ \bar e_{ij} \bar e_{lj} }} }^2 = \bigO{\frac{1}{qT}}, \\
                & \EE\abs{ \frac{1}{pT} \sum_{t=1 }^{T} \sum_{i=1}^{p} \paran{e_{t, ij} e_{t, ih} - \E{ e_{t, ij} e_{t, ih} }} }^2 = \bigO{\frac{1}{pT}},
                & \EE\abs{ \frac{1}{p} \sum_{i=1}^{p} \paran{\bar e_{ij} \bar e_{ih} - \E{ \bar e_{ij} \bar e_{ih} }} }^2 = \bigO{\frac{1}{pT}},  \\
                & \EE \norm{ \frac{1}{p q T} \sum_{t=1}^{T} \bE_t \bE_t^\top - \frac{1}{p q T} \E{ \sum_{t=1}^{T} \bE_t \bE_t^\top } }_F^2 = \bigO{ \frac{1}{qT} },
                & \EE \norm{ \frac{1}{p q} \bar\bE \bar\bE^\top - \frac{1}{p q T} \E{ \bar\bE \bar\bE^\top } }_F^2 = \bigO{ \frac{1}{qT} }, \\
                & \EE \norm{ \frac{1}{p q T} \sum_{t=1}^{T} \bE_t^\top \bE_t - \frac{1}{p q T} \E{ \sum_{t=1}^{T} \bE_t^\top \bE_t } }_F^2 = \bigO{ \frac{1}{pT} },
                & \EE \norm{ \frac{1}{p q} \bar\bE^\top \bar\bE  - \frac{1}{p q} \E{ \bar\bE^\top \bar\bE } }_F^2 = \bigO{ \frac{1}{pT} }.
            \end{aligned}
        \end{equation}

        By Davydov's inequality (Corollary 16.2.4 in \cite{athreya2006measure}), there is a constant $C>0$, for all $i,l \in [p]$, $j,h \in [q]$, and $s, t \in [T]$, $\abs{ \Cov{e_{t, ij} e_{t, lh}, e_{s, ij} e_{s, lh}}} = \bigO{1} \alpha( \abs{t-s} )^{1 - 2/\gamma}$.
        Under $\alpha$-mixing Assumption \ref{assume:alpha-mixing}, we have $\sum_{ h > 1 } \alpha( h )^{1 - 2/\gamma} = \bigO{1}$.
       We have,  for any row $i$ and $l$,
       \begin{equation*}
           \begin{aligned}
               & \E{ \frac{1}{qT} \sum_{t=1}^{T} \sum_{j=1}^{q} \paran{ e_{t, ij} e_{t, lj} - \E{ e_{t, ij} e_{t, lj} } } }^2 \\
               & =  \frac{1}{q^2T^2} \paran{ \sum_{t=1}^{T} \sum_{j=1}^{q} \Cov{e_{t, ij} e_{t, lj}, e_{t, ij} e_{t, lj}} }
               + \frac{1}{q^2T^2} \paran{ \sum_{t=1}^T \sum_{j=1}^{q} \sum_{ s \ne t }  \Cov{e_{t, ij} e_{t, lj}, e_{s, i j} e_{s, l j}} }  \\
               & + \frac{1}{q^2T^2} \paran{ \sum_{t=1}^{T} \sum_{j=1}^{q} \sum_{h \ne j} \Cov{ e_{t, ij} e_{t, lj}, e_{t, ih} e_{t, lh}  } }
               + \frac{1}{q^2T^2} \paran{ \sum_{t=1}^{T} \sum_{j=1}^{q}  \sum_{ s \ne t } \sum_{h \ne j} \Cov{ e_{t, ij} e_{t, lj}, e_{s, ih} e_{s, lh}  } }  \\
               % & = \bigO{\frac{1}{qT} + \frac{1}{qT^2} + \frac{1}{q^2T} + \frac{1}{q^2T^2}}    \\
               & = \bigO{\frac{1}{qT}},
           \end{aligned}
       \end{equation*}
        where we also used Assumption \ref{assume:cross_row_col_corr} (d) on weak row-/column-wise correlation of $\bE_t$ to bound the last two terms.
        Similarly for columns $j$ and $h$, we have
        \[
        \E{ \frac{1}{pT} \sum_{t=1 }^{T} \sum_{i=1}^{p} \paran{e_{t, ij} e_{t, ih} - \E{ e_{t, ij} e_{t, ih} }} }^2 = \bigO{\frac{1}{pT}}.
        \]
        % Then, from Markov inequality, we obtain the desired results.

        Next, we have
        \begin{equation*}
            \begin{aligned}
                \EE\abs{ \frac{1}{q} \sum_{j=1}^{q} \paran{\bar e_{ij} \bar e_{lj} - \E{ \bar e_{ij} \bar e_{lj} }} }^2 & =  \EE\abs{ \frac{1}{q T^2} \sum_{j=1}^{q} \sum_{t=1}^{T} \sum_{s=1}^{T} \paran{ e_{t,ij} e_{s,lj} - \E{e_{t,ij} e_{s,lj}}} }^2 \\
                & \le \frac{1}{T}\sum_{s=1}^{T}  \E{ \paran{\frac{1}{q T} \sum_{j=1}^{q} \sum_{t=1}^{T} \paran{ e_{t,ij} e_{s,lj} - \E{e_{t,ij} e_{s,lj}}} }^2 } \\
                &= \bigO{\frac{1}{qT}}.
            \end{aligned}
        \end{equation*}
       Similarly, we can show that $\EE\abs{ \frac{1}{p} \sum_{i=1}^{p} \paran{\bar e_{ij} \bar e_{ih} - \E{ \bar e_{ij} \bar e_{ih} }} }^2 = \bigO{\frac{1}{pT}}$.

        Finally, we have
        \begin{equation*}
            \E{ \norm{ \frac{1}{p q T} \sum_{t=1}^{T} \bE_t \bE_t^\top - \frac{1}{p q T} \E{ \sum_{t=1}^{T} \bE_t \bE_t^\top } }_F^2 }
            = \E{ \frac{1}{p^2} \sum_{i=1}^{p} \sum_{l=1}^{p} \paran{ \frac{1}{qT} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, ij} e_{t, lj} - \E{ e_{t, ij} e_{t, lj} } }^2 }
            = \bigO{\frac{1}{qT}}. \nonumber
        \end{equation*}
        The remaining results follow by a similar argument.
        %Then, the result follows from Markov inequality.

     %\item  The proofs are the same as that of \ref{cond:moments_CLT}.1 and are thus omited. % \ref{cond:moments_CLT}.3, \ref{cond:moments_CLT}.4

    \underline{\sc Step 2.} Following the same argument as that of \underline{\sc Step 2} of Lemma \ref{assume:moments_0}, we can show the final results of Lemma \ref{assume:moments_Et_0}.


    \item
    \underline{\sc Step 1.} We firstly prove that, for all $1 \le t \le T$, $\mathbb{E} \, \norm{ \frac{1}{\sqrt{pq}} \bR \bE_t \bC^\top }^2 =\bigO{1}$.

    We have,
    \begin{equation*}
    \begin{aligned}
    \mathbb{E} \, \norm{ \frac{1}{\sqrt{pq}} \bR \bE_t \bC^\top }^2
    & = \mathbb{E} \, \norm{ \frac{1}{\sqrt{pq}} \sum_{i=1}^p \sum_{j=1}^q \bR_{i\cdot}\bC_{j\cdot}^\top e_{t,ij}}^2 = \bigO{1},
    \end{aligned}
    \end{equation*}
which follows from Assumption \ref{assume:CLT}.

    \underline{\sc Step 2.} Next, we have, for all $1 \le t \le T$,
    \begin{eqnarray*}
        \mathbb{E}\,\norm{ \frac{1}{\sqrt{pq}} \bR \tilde\bE_t \bC^\top }^2 & \le & \mathbb{E}\,\norm{ \frac{1}{\sqrt{pq}} \bR \bE_t \bC^\top }^2 + \tilde\alpha\mathbb{E}\,\norm{ \frac{1}{\sqrt{pq}} \bR \bar\bE_t \bC^\top}^2 \le \paran{1+\tilde\alpha}\mathbb{E}\,\norm{ \frac{1}{\sqrt{pq}} \bR \bE_t \bC^\top }^2 = \bigO{1}.
    \end{eqnarray*}

     \begin{comment}
     Denote $\bA_t = \frac{1}{\sqrt{pq}} \bR \bE_t \bC^\top$, we have $\E{\bA_t}=\bzero$ and  $\E{\norm{\bA_t}^2} = \bigO{1}$ from \ref{cond:moments_CLT}.3.
     By Assumption \ref{assume:alpha-mixing}, we have $\vect{\bA_t}$ and $\vect{\bF_t}$ are both $\alpha$-mixing.
     Then,
     \begin{equation*}
     \begin{aligned}
     \mathbb{E}\,\norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \bR^\top \bE_t\bC \bF_t^\top}^2 & = \mathbb{E}\,\norm{ \frac{1}{\sqrt{T}} \sum_{t=1}^{T} \bA_t \bF_t }^2
     \end{aligned}
     \end{equation*}
     \end{comment}

    \end{enumerate}
    % $\sum_{j \ne h} \Cov{ e_{t, ij} e_{t, lj}, e_{t, ih} e_{t, lh} } = \Op{1}$
    % $\sum_{i \ne l} \Cov{ e_{t, ij} e_{t, ih}, e_{t, lj} e_{t, lh} } = \Op{1}$
    % $\sum_{ t \ne s } \sum_{j \ne h} \Cov{ e_{t, ij} e_{t, lj} e_{s, ih} e_{s, lh} } = \Op{1}$
\end{proof}


\paragraph{Proof of Lemma \ref{assume:CLT_0}.}
\begin{proof}~
\begin{enumerate}[label=(\alph*)]
    \item
    \underline{\sc Step 1.} We firstly prove \eqref{eqn:lemma-clt-1} stated as follows.


    For each row $i\in[p]$, as $q, T \rightarrow \infty$,
    \begin{equation} \label{eqn:lemma-clt-1}
    \begin{pmatrix}
        \frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \bF_t \bC^\top \be_{t, i \cdot} \\
        \frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \bC^\top \be_{t, i \cdot}
    \end{pmatrix}
    \convdist
    \calN \paran{
       \bzero, \begin{pmatrix}
            \bPhi_{R, i, 11} & \bPhi_{R, i, 12} \\
            \bPhi_{R, i, 21} & \bPhi_{R, i, 22}
    \end{pmatrix}
    }.
    \end{equation}


     For any $i\in[p]$ and $t\in [T]$, we define a random vector $\bx_t = \frac{1}{\sqrt{q}} \sum_{j=1}^q \bC_{j\cdot} e_{t, i j}$, which is $\alpha$-mixing over $t$.
     By Assumption \ref{assume:factor-noise-matrix}, we have $\E{\bF_t\bx_t} = 0$ and $\E{\bx_t} = 0$.
     We rewrite
     \begin{equation*}
         \begin{aligned}
              \begin{pmatrix}
                 \frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \bF_t \bC^\top \be_{t, i \cdot} \\
                 \frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \bC^\top \be_{t, i \cdot}
              \end{pmatrix}
            & = \frac{1}{\sqrt{T}} \sum_{t=1}^{T}
               \begin{pmatrix} \bF_t \\ \bI_r \end{pmatrix} \bx_t.
         \end{aligned}
     \end{equation*}

      In order to apply the central limit theorem for $\alpha$-mixing data \cite[Theorem 2.21]{fan2008nonlinear}, we need to show that there exists an $m>2$ such that $\E{\norm{\begin{pmatrix} \bF_t^\top & \bI_r \end{pmatrix}^\top \bx_t}^m} \le C$.
      Since $\bF_t$ is of fixed dimensions, it suffices to show that $\E{\paran{\bff_{t,l\cdot}^\top\bx_t}^m} \le C$ and $\E{x_{t,h}^m} \le C$ for any $l\in [k]$ and $h \in [r]$.

      By Holder inequality, we have for any $1< a, b < \infty$ and $1/a + 1/b = 1$,
      \begin{equation*}
      \E{\paran{\bff_{t,l\cdot}^\top\bx_t}^m}
      \le \E{\norm{\bff_{t,l\cdot}}^m \norm{\bx_t}^m}
      \le \paran{ \E{\norm{\bff_{t,l\cdot}}^{ma} } }^{1/a} \paran{\E{\norm{\bx_t}^{mb}}}^{1/b}.
      \end{equation*}
      By Assumption \ref{assume:CLT}, we have $\E{\paran{\bff_{t,l\cdot}^\top\bx_t}^m} \le C$ for any $l\in [k]$. Similarly, we have $\E{x_{t,h}^m} \le C$ for any $h \in [r]$.
      Then Theorem 2.21 in \cite{fan2008nonlinear} implies the desired result.

      \underline{\sc Step 2.} Now we show the final results of Lemma \ref{assume:CLT_0} (a).

      Plugging in $\tilde e_{t, ij} \defeq e_{t, ij} + \tilde\alpha \bar e_{ij}$, $\tilde \bF_t \defeq \bF_t + \tilde\alpha \bar\bF$ and using the fact that $2\tilde\alpha + \tilde\alpha^2 = \alpha$,  we have
            \begin{eqnarray}
                \frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \tilde \bF_t \bC^\top \tilde\be_{t, i \cdot}
                & = & \frac{\sqrt{T}}{\sqrt{q}} \frac{1}{T} \sum_{t=1}^{T} \paran{\bF_t + \tilde a \, \bar\bF} \bC^\top \paran{\be_{t, i \cdot} + \tilde a \, \bar\be_{i \cdot}} \nonumber \\
                & = & \begin{pmatrix} \bI_k & \alpha \bar\bF \end{pmatrix}
                \begin{pmatrix}
                    \frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \bF_t \bC^\top \be_{t, i \cdot} \\
                    \frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \bC^\top \be_{t, i \cdot}
                \end{pmatrix}.
                \nonumber
            \end{eqnarray}

            By \eqref{eqn:lemma-clt-1} and continuous mapping theorem, we have for each row $i$, as $q, T \rightarrow \infty$,
            \[
            \frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \tilde\bF_t \bC^\top \tilde\be_{t, i \cdot}
            \convdist
            \calN \paran{\bzero,
                \begin{pmatrix} \bI_k & \alpha \bmu_F \end{pmatrix}
                \begin{pmatrix}
                    \bPhi_{R, i, 11} & \bPhi_{R, i, 12} \\
                    \bPhi_{R, i, 21} & \bPhi_{R, i, 22}
                \end{pmatrix}
                \begin{pmatrix} \bI_k \\ \alpha \bmu_F^\top \end{pmatrix}
            }.
            \]


    \item \underline{\sc Step 1.} Following the same argument as in that in (a), we have that for each column $j$, as $p, T \rightarrow \infty$,
    \begin{equation} \label{eqn:lemma-clt-2}
        \begin{pmatrix}
            \frac{1}{\sqrt{pT}} \sum_{t=1}^{T} \bF_t^\top \bR^\top \be_{t, \cdot j }  \\
            \frac{1}{\sqrt{pT}} \sum_{t=1}^{T} \bR^\top \be_{t, \cdot j}
        \end{pmatrix} \convdist \calN \paran{ \bzero, \begin{pmatrix}
                \bPhi_{C, j, 11} & \bPhi_{C, j, 12} \\
                \bPhi_{C, j, 21} & \bPhi_{C, j, 22}
        \end{pmatrix} },
    \end{equation}

    \underline{\sc Step 2.} Now we show the final results of Lemma \ref{assume:CLT_0} (b).

    Plugging in $\tilde e_{t, ij} \defeq e_{t, ij} + \tilde\alpha \bar e_{ij}$, $\tilde \bF_t \defeq \bF_t + \tilde\alpha \bar\bF$ and using the fact that $2\tilde\alpha + \tilde\alpha^2 = \alpha$,  we have
            \begin{eqnarray}
                \frac{1}{\sqrt{pT}} \sum_{t=1}^{T} \tilde\bF_t^\top \bR^\top \tilde\be_{t, \cdot j } & = & \frac{\sqrt{T}}{\sqrt{p}} \frac{1}{T} \sum_{t=1}^{T} \paran{\bF_t + \tilde a \, \bar\bF}^\top \bR^\top \paran{\be_{t, \cdot j} + \tilde a \, \bar\be_{\cdot j}} \nonumber \\
                & = & \begin{pmatrix} \bI_r & \alpha \bar\bF^\top \end{pmatrix}
                \begin{pmatrix}
                    \frac{1}{\sqrt{pT}} \sum_{t=1}^{T} \bF_t^\top \bR^\top \be_{t, \cdot j }  \\
                    \frac{1}{\sqrt{pT}} \sum_{t=1}^{T} \bR^\top \be_{t, \cdot j}
                \end{pmatrix}. \nonumber
            \end{eqnarray}

            By \eqref{eqn:lemma-clt-2} and continuous mapping theorem, we have for each column $j$, as $p, T \rightarrow \infty$,
            \[
            \frac{1}{\sqrt{pT}} \sum_{t=1}^{T} \tilde\bF_t^\top \bR^\top \tilde\be_{t, \cdot j }
            \convdist
            \calN \paran{\bzero,
                \begin{pmatrix} \bI_r & \alpha \bmu_F^\top \end{pmatrix}
                \begin{pmatrix}
                    \bPhi_{C, j, 11} & \bPhi_{C, j, 12} \\
                    \bPhi_{C, j, 21} & \bPhi_{C, j, 22}
                \end{pmatrix}
                \begin{pmatrix} \bI_r \\ \alpha \bmu_F \end{pmatrix}
            }.
            \]

    \end{enumerate}
\end{proof}



==> proofs.tex <==

%!TEX root = 0-main.tex

\section{Proofs} \label{sec:proof}

%%----------------------------------------
%%
%% assumption altered for local use
%%
\newtheorem{assumptionalter}{Lemma}
\renewcommand*{\theassumptionalter}{\Alph{assumptionalter}0}

%%
%% ----------------------------------------

We establish the convergence and asymptotic normality of the estimator based on equation \eqref{eqn:M-tildeY}, under Assumption \ref{assume:alpha-mixing} - \ref{assume:CLT} in the main text.

\subsection{Useful lemmas}

We first present lemmas on $\tilde\bY_t$, $\tilde\bF_t$, and $\tilde\bE_t$ under Assumption \ref{assume:alpha-mixing} - \ref{assume:CLT}.
These results will be used to prove main theorems.
The proofs are delayed to Section \ref{sec:proof-B}.

\begin{lemma} \label{assume:factor_matrix_0}
Under Assumption \ref{assume:alpha-mixing} - \ref{assume:cross_row_col_corr},
we have
$\E{\norm{\tilde\bF_t}^4} \le C < \infty$.
As $T \rightarrow \infty$, we have that,
\begin{equation*}
    \frac{1}{qT}\sum_{t=1}^T\tilde\bF_t \bC^\top\bC \tilde\bF_t^\top \convprob \tilde\bSigma_{FC} , \quad\text{and}\quad \frac{1}{pT}\sum_{t=1}^T\tilde\bF_t^\top\bR^\top\bR\tilde\bF_t \convprob \tilde\bSigma_{FR}.
\end{equation*}
where $\tilde\bSigma_{FC} = \bSigma_{FC} + \paran{1+\alpha} \bmu_F (\bC^\top\bC/q) \bmu_F^\top$, $\tilde\bSigma_{FR} = \bSigma_{FR} + \paran{1+\alpha} \bmu_F (\bR^\top\bR/p) \bmu_F^\top$, $\bSigma_{FC}$ and $\bSigma_{FR}$ are defined in \eqref{eqn:Sigma_FC_FR}.
\end{lemma}

\begin{lemma}\label{assume:cross_row_col_corr_0}
Under Assumption \ref{assume:alpha-mixing} - \ref{assume:cross_row_col_corr},
we have that here exists a positive constant $C < \infty$ such that for all $N$ and $T$,
    \begin{enumerate}[label=(\alph*)]
        \item For all $i \in [p]$, $j \in [q]$ and $t \in [T]$, $\E{\tilde e_{t, ij}} = 0$ and $\EE \lvert \tilde e_{t, ij} \rvert^8 \le C$.

        \item Let  $\tilde\bU_E = \E{\frac{1}{qT} \sum_{t=1}^{T} \tilde\bE_t \tilde\bE_t^T}$ and $\tilde\bV_E = \E{\frac{1}{pT} \sum_{t=1}^{T} \tilde\bE_t^T \tilde\bE_t}$, we assume
        \begin{equation*}
            \norm{ \tilde\bU_E }_1 \le C, \quad \norm{ \tilde\bV_E }_1 \le C.
        \end{equation*}
    \end{enumerate}
\end{lemma}


\begin{lemma} \label{assume:temporal_dependence_0}
Under Assumption \ref{assume:alpha-mixing} - \ref{assume:CLT},
we have
\begin{equation*}
    \sum_{s=1}^{T} \norm{ \E{ \frac{1}{p q} \bR^\top \tilde\bE_s \tilde\bE_t^\top \bR } }_2 = \bigO{1}, \qquad
    \sum_{s=1}^{T} \norm{ \E{ \frac{1}{p q} \bC^\top \tilde\bE_s^\top \tilde\bE_t \bC} }_2 = \bigO{1}.
\end{equation*}
\end{lemma}


\begin{lemma} \label{assume:factor_noise_weak_corr_0}
Under Assumption \ref{assume:alpha-mixing} - \ref{assume:CLT},
For any $i\in [p]$ and $j \in [q]$,
\begin{equation*}
    \begin{aligned}
%        & \E{\norm{\frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \tilde e_{t, ij} \tilde \bF_{t}}^2} = \bigO{1}, \qquad
%        \E{\norm{\frac{1}{\sqrt{p T}} \sum_{t=1}^{T} \sum_{i=1}^{p} \tilde e_{t, ij} \tilde \bF_{t}}^2} = \bigO{1}, \\
        & \E{\norm{\frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \tilde \bF_{t} \bC^\top \tilde  \be_{t, i \cdot}}^2} = \bigO{1}, \qquad
        \E{\norm{\frac{1}{\sqrt{p T}} \sum_{t=1}^{T} \tilde \bF_{t}^\top \bR^\top \tilde \be_{t, \cdot j}}^2} = \bigO{1},
    \end{aligned}
\end{equation*}
% For any $l\in [p]$, $\norm{ \frac{1}{ \sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, lj} \bC_{j \cdot}^\top \bF_t^\top }^2 = \Op{1}$.
\end{lemma}



\begin{lemma} \label{assume:moments_0}
Under Assumption \ref{assume:alpha-mixing} - \ref{assume:CLT},
we have
\begin{enumerate}[label=(\alph*)]
    \item For any row $i\in[p]$,
    \[
    \mathbb{E} \paran{ \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( \tilde e_{t, lj} \tilde e_{t, ij} - \E{\tilde e_{t, lj} \tilde e_{t, ij}} \right)}^2  = \bigO{1}.
    \]
    Similarly, for any column $j\in[q]$,
     \[
    \mathbb{E} \paran{ \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{i=1}^{p} \sum_{h=1}^{q} \left( \tilde e_{t, ih} \tilde e_{t, ij} - \E{ \tilde e_{t, ih} \tilde e_{t, ij}} \right)}^2  = \bigO{1}.
    \]
    \item The $k \times k$ matrix satisfies
    \[
    \mathbb{E}\,\norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \bR^\top \tilde\bE_t \bC \tilde\bF_t^\top}^2 = \bigO{1}.
    \]
    Similarly, the $r \times r$ matrix satisfies
    \[
    \mathbb{E} \, \norm{\frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \tilde\bF_t^\top \bR^\top \tilde\bE_t \bC }^2 = \bigO{1}.
    \]
    \end{enumerate}
\end{lemma}

\begin{lemma}  \label{assume:moments_Et_0}
Under Assumption \ref{assume:alpha-mixing} - \ref{assume:CLT}, we have for all $p$, $q$ and $T$,
    \begin{enumerate}[label=(\alph*)]
        \item For any $i,l \in [p]$ and $j,h \in [q]$,
        \begin{equation*}
            \begin{aligned}
                & \EE\paran{ \frac{1}{\sqrt{qT}} \sum_{t=1 }^{T} \sum_{j=1}^{q} \paran{\tilde e_{t, ij} \tilde e_{t, lj} - \E{ \tilde e_{t, ij} \tilde e_{t, lj} }} }^2 = \bigO{1},  \quad
                \EE\paran{ \frac{1}{\sqrt{pT}} \sum_{t=1 }^{T} \sum_{i=1}^{p} \paran{\tilde e_{t, ij} \tilde e_{t, ih} - \E{ \tilde e_{t, ij} \tilde e_{t, ih} }} }^2 = \bigO{1},\\
                & \EE \norm{ \frac{1}{p \sqrt{q T}} \sum_{t=1}^{T} \paran{\tilde\bE_t \tilde\bE_t^\top - \E{  \tilde\bE_t \tilde\bE_t^\top } } }_F^2 = \bigO{ 1 },  \quad
                \EE \norm{ \frac{1}{p \sqrt{q T}} \sum_{t=1}^{T} \paran{\tilde\bE_t^\top \tilde\bE_t - \E{ \tilde\bE_t^\top \tilde\bE_t } } }_F^2 = \bigO{ 1 }.
            \end{aligned}
        \end{equation*}

        \item For all $1 \le t \le T$,
        $\mathbb{E} \, \norm{ \frac{1}{\sqrt{pq}} \bR \tilde\bE_t \bC^\top }^2 =\bigO{1}$.
    \end{enumerate}
\end{lemma}

\begin{lemma}\label{assume:CLT_0}
Under Assumption \ref{assume:alpha-mixing} - \ref{assume:CLT}, we have
\begin{enumerate}[label=(\alph*)]
    \item For each row $i$, as $q, T \rightarrow \infty$,
    \[
    \frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \tilde\bF_t \bC^\top \tilde\be_{t, i \cdot}
    \convdist
    \calN \paran{\bzero,
        \begin{pmatrix} \bI_k & \alpha \bmu_F \end{pmatrix}
        \begin{pmatrix}
            \bPhi_{R, i, 11} & \bPhi_{R, i, 12} \\
            \bPhi_{R, i, 21} & \bPhi_{R, i, 22}
        \end{pmatrix}
        \begin{pmatrix} \bI_k \\ \alpha \bmu_F^\top \end{pmatrix}
    }.
    \]
    \item For each column $j$, as $p, T \rightarrow \infty$,
    \[
    \frac{1}{\sqrt{pT}} \sum_{t=1}^{T} \tilde\bF_t^\top \bR^\top \tilde\be_{t, \cdot j }
     \convdist
    \calN \paran{\bzero,
        \begin{pmatrix} \bI_r & \alpha \bmu_F^\top \end{pmatrix}
        \begin{pmatrix}
            \bPhi_{C, j, 11} & \bPhi_{C, j, 12} \\
            \bPhi_{C, j, 21} & \bPhi_{C, j, 22}
        \end{pmatrix}
        \begin{pmatrix} \bI_r \\ \alpha \bmu_F \end{pmatrix}
    }.
    \]
    The $\bPhi_{R, i, \cdot\cdot}$'s and $\bPhi_{C, j, \cdot\cdot}$'s are defined in Theorem \ref{thm:asymp normality of R/C}. % \eqref{eqn:lemma-clt-1}, \eqref{eqn:lemma-clt-2}
\end{enumerate}
\end{lemma}


\subsection{A high-level summary of proofs}

%The main purpose is to avoid tracking $\alpha$ in the majority of the proof.
In the remaining part of Section \ref{sec:proof}, we use $\bY_t$, $\bF_t$, and $\bE_t$ in place for $\tilde\bY_t$, $\tilde\bF_t$, and $\tilde\bE_t$ to improve the readability of the proofs.
Our estimator $\hat \bR$ ($\hat \bC$) is then given by the matrix of $\sqrt{p}$ ($\sqrt{q}$) times the top $k$ ($r$) eigenvectors of $\hat \bM_R \; \defeq \; \frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top$ ($\hat \bM_C \; \defeq \; \frac{1}{p q T} \sum_{t = 1}^{T} \bY_t^\top \bY_t$) in descending order by corresponding eigenvalues.
%The first objective is to derive the asymptotic normality of each row of $\hbR$ and $\hbC$.
Recall that some auxiliary matrices $\bV_{R, pqT}$, $\bV_{C, pqT}$, $\bH_C$ and $\bH_R$ are defined as following.

Let $\bV_{R, pqT} \in \RR^{k \times k}$ and $\bV_{C, pqT} \in \RR^{r \times r}$ be the diagonal matrices consisting of the first $k$ and $r$ largest eigenvalues of $\frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top$ and $\frac{1}{p q T} \sum_{t = 1}^{T} \bY_t^\top \bY_t$ in decreasing order, respectively.
By definition of eigenvectors and eigenvalues, we have
$$\frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top \hbR = \hbR \bV_{R, pqT}, \quad \text{or} \quad \hbR = \frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top \hbR \bV_{R, pqT}^{-1},$$
$$\frac{1}{p q T} \sum_{t = 1}^{T} \bY_t^\top \bY_t \hbC = \hbC \bV_{C, pqT}, \quad \text{or} \quad \hbC = \frac{1}{p q T} \sum_{t = 1}^{T} \bY_t^\top \bY_t \hbC \bV_{C, pqT}^{-1}.$$

Define $\bH_R \in \RR^{k \times k}$ and $\bH_C \in \mathbb{R}^{r \times r}$ as
\begin{eqnarray}
\bH_R = \frac{1}{p q T} \sum_{t=1}^{T} \bF_t \bC^\top \bC \bF_t^\top \bR^\top \hbR \bV_{R, pqT}^{-1} \in \mathbb{R}^{k \times k} \nonumber \\
\bH_C = \frac{1}{p q T} \sum_{t=1}^{T} \bF_t^\top \bR^\top \bR \bF_t \bC^\top \hbC \bV_{C, pqT}^{-1} \in \mathbb{R}^{r \times r}. \nonumber
\end{eqnarray}

Then we have
\begin{eqnarray} \label{eqn:proof:hatR-RH}
	\hbR - \bR \bH_R & = & \frac{1}{p q T} \left( \sum_{t = 1}^{T} \bY_t^\top \hbR  - \bR \sum_{t = 1}^{T} \bF_t \bC^\top \bC \bF_t^\top \bR^\top \hbR  \right) \bV_{R, pqT}^{-1}  \\
	& = & \left(  \frac{1}{p q T} \sum_{t=1}^{T} \bR  \bF_t \bC^\top \bE_t^\top \hbR  + \frac{1}{p q T} \sum_{t=1}^{T} \bE_t \bC \bF_t^\top \bR^\top \hbR  + \frac{1}{p q T} \sum_{t=1}^{T} \bE_t \bE_t^\top \hbR \right) \bV_{R, pqT}^{-1}, \nonumber
\end{eqnarray}
and
\begin{eqnarray} \label{eqn:proof:hatC-CH}
\hbC - \bC \bH_C & = & \frac{1}{p q T} \left( \sum_{t=1}^{T} \bY_t^\top \bY_t \hbC  - \bC \sum_{t=1}^{T} \bF_t^\top \bF_t \bC^\top \hbC  \right) \bV_{C, pqT}^{-1}  \\
& = & \left( \frac{1}{p q T} \sum_{t=1}^{T} \bC \bF_t^\top \bR^\top \bE_t \hbC  + \frac{1}{p q T} \sum_{t=1}^{T} \bE_t^\top \bR \bF_t \bC^\top \hbC  + \frac{1}{p q T} \sum_{t=1}^{T} \bE_t^\top \bE_t \hbC \right) \bV_{C, pqT}^{-1} \nonumber
\end{eqnarray}

Our objective is to derive the asymptotic normality of $\hbR_{i \cdot} - \bH_R^\top \bR _{i \cdot}$ ($\hbC_{j \cdot} - \bH_C^\top \bC _{i \cdot}$) -- each row of $\hbR$ ($\hbC$). We now describe the structure of the proofs for $\hbR_{i \cdot} - \bH_R^\top \bR _{i \cdot}$.
\begin{enumerate}
    \item In Section \ref{sec:proof F norm}, we bound $\frac{1}{p}\norm{\hbR - \bR \bH_R}^2_F$.
    \item In Section \ref{sec:proof Rhat R}, we derive the asymptotic behavior of ${\hbR^\top \bR }/{p}$ and ${\hbC^\top \bC }/{q}$.
    \item In Section \ref{sec:proof Rhat R}, we derive the asymptotic behavior of $\bV_{R, pqT}$, $\bV_{C, pqT}$, $\bH_C$ and $\bH_R$.
    \item In Section \ref{sec:proof for R}, we derive the asymptotic distributions.
    The idea is to first bound $\frac{1}{p}\norm{\hbR - \bR \bH_R}^2_F$ and then derive asymptotic distribution for each row $\hbR_{i \cdot} - \bH_R^\top \bR_{i \cdot} $ for $i \in [p]$.
    Results for $\hbC_{j \cdot} - \bH_C^\top \bC_{j \cdot} $ for $1 \le j \le q$ are derived analogously with $\frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top$.
    \item In Section \ref{sec:proof F_t}, we analyze the convergence rate for $\hat \bF_t$, $1 \le t \le T$.
\end{enumerate}
%Assume $\frac{1}{p} \hbR' \hbR = \bI_{k}$, then the columns of $\hbR$ compose of the eigenvectors of $\frac{1}{p q T} \sum_{t = 1}^{T} \bS_t \bS_t^\top$.
%However, we can only observe $\bY_t = \bS_t + \bE_t$.
%Estimator $\hbR$ is obtained as the matrix whose columns are the eigenvectors of $\frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top$ corresponding to its largest $k$ eigenvalues.


\subsection{Theorem \ref{thm:Rhat_F_norm_convg}: \texorpdfstring{$\hbR$ and $\hbC$}{hat R and hat C} converge in Frobenius and \texorpdfstring{$\ell_2$-norm}{L2 norm}} \label{sec:proof F norm}

In the remaining part of Section \ref{sec:proof}, we use $\bY_t$, $\bF_t$, and $\bE_t$ in place for $\tilde\bY_t$, $\tilde\bF_t$, and $\tilde\bE_t$ to improve the readability of the proofs.

%\textcolor{red}{Double checked. Right!}
\begin{lemma}  \label{thm:lemma-3terms}
    Under Assumption \ref{assume:alpha-mixing} - \ref{assume:CLT}, we have
    \begin{eqnarray}
        \norm{\sum_{t=1}^{T} \bF_t \bC^\top \bE_t^\top}_F^2 & = &  \norm{\sum_{t=1}^{T} \bE_t \bC \bF_t^\top }_F^2 = \Op{p q T} \nonumber \\
        \norm{\sum_{t=1}^{T} \bE_t \bE_t^\top}_F^2 & =  & \Op{p^2 q T} + \Op{p q^2 T^2} \nonumber
    \end{eqnarray}
\end{lemma}

\begin{proof}
    We have $\bF_t \bC^\top \bE_t^\top = \paran{\bE_t \bC \bF_t^\top}^\top$, so their Frobenius norms are the same.
    Expanding each terms, we have
    \begin{eqnarray}
        \norm{\sum_{t=1}^{T} \bF_t \bC^\top \bE_t^\top}_F^2 & = & \norm{\sum_{t=1}^{T} \sum_{j=1}^{q} \bF_t \bC_{j \cdot} \be_{t, \cdot j}^\top}_F^2 = q T \norm{\frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \left( \be_{t, \cdot j} \otimes \bF_t \right) \bC_{j \cdot} }^2 \nonumber \\
        & = & q T \sum_{i=1}^{p} \norm{\frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, ij} \bF_t \bC_{j \cdot} }^2 \nonumber \\
        & = & \Op{p q T},  \nonumber
    \end{eqnarray}
    where the final results is obtained by Lemma  \ref{assume:factor_noise_weak_corr_0} and Markov inequality.

    Thus, we have $\norm{\sum_{t=1}^{T} \bF_t \bC^\top \bE_t^\top}_F^2 = \Op{1}$.
    \begin{eqnarray}
        \norm{\sum_{t=1}^{T} \bE_t \bE_t^\top}_F^2 & = & \norm{ \sqrt{qT}  \frac{\sum_{t=1}^{T} \sum_{j=1}^{q} \be_{t, \cdot j} \be_{t, \cdot j}^\top}{\sqrt{qT}}}_F^2 \nonumber \\
        & = & q T  \sum_{i=1}^{p} \sum_{l=1}^{p} \norm{ \frac{\sum_{t=1}^{T} \sum_{j=1}^{q}  e_{t, ij} e_{t, lj}}{ \sqrt{qT} } }^2 \nonumber \\
        & \le & p^2 q T \cdot \frac{1}{p^2}  \sum_{i=1}^{p} \sum_{l=1}^{p} \norm{\frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \left( e_{t, ij} e_{t, lj} - \E{e_{t, ij} e_{t, lj}} \right)}^2 \nonumber \\
        & & +  p q^2 T^2 \cdot \frac{1}{p} \sum_{i=1}^{p} \paran{ \sum_{l=1}^{p}  \norm{ \E{ \frac{\sum_{t=1}^{T} \sum_{j=1}^{q}  e_{t, ij} e_{t, lj}}{q T}} }^2 }  \nonumber \\
        & = & \Op{p^2 q T } + \bigO{p q^2 T^2 }, \nonumber
    \end{eqnarray}
    where the last equality follows from Lemma \ref{assume:moments_Et_0} (a) and Lemma \ref{assume:cross_row_col_corr_0} (b).
\end{proof}


\noindent\textbf{Proof of Theorem \ref{thm:Rhat_F_norm_convg}}
\begin{proof}
    Consider each term in equation \eqref{eqn:proof:hatR-RH},  we have
    \begin{eqnarray}
        \frac{1}{p^3 q^2 T^2} \norm{\sum_{t=1}^{T} \bR  \bF_t \bC^\top \bE_t^\top \hbR}_F^2  & \le & \frac{1}{p^3 q^2 T^2} \norm{\bR}_F^2 \norm{\sum_{t=1}^{T} \bF_t \bC^\top \bE_t^\top}_F^2 \norm{\hbR}_F^2 = \Op{ \frac{1}{q T} }, \nonumber \\
        \frac{1}{p^3 q^2 T^2} \norm{\sum_{t=1}^{T} \bE_t \bC \bF_t^\top \bR^\top \hbR}_F^2 & \le & \frac{1}{p^3 q^2 T^2} \norm{\sum_{t=1}^{T} \bE_t \bC \bF_t^\top}_F^2 \norm{\bR^\top}_F^2 \norm{\hbR }_F^2 = \Op{ \frac{1}{q T}}, \nonumber \\
        \frac{1}{p^3 q^2 T^2} \norm{ \sum_{t=1}^{T} \bE_t \bE_t^\top \hbR }_F^2  & \le & \frac{1}{p^3 q^2 T^2} \norm{\sum_{t=1}^{T} \bE_t \bE_t^\top}_F^2 \norm{\hbR }_F^2 = \Op{ \frac{1}{q T}} + \Op{ \frac{1}{p}}, \nonumber
    \end{eqnarray}
    where the last equality of each equation results from Lemma \ref{thm:lemma-3terms}. Combing them together, we have
    \[
    \frac{1}{p}\norm{\hbR - \bR \bH_R}^2_F = \Op{\frac{1}{p} + \frac{1}{qT}}.
    \]
    Result for $\hbC$ is derived from equation \eqref{eqn:proof:hatC-CH} in a similar fashion.
    Note that
    $$\frac{1}{k}\norm{\hat \bR - \bR \bH_R}^2_F \le \norm{\hat \bR - \bR \bH_R}^2 \le \norm{\hat \bR - \bR \bH_R}^2_F.$$
    We also have
    \[\frac{1}{p} \norm{\hat \bR - \bR \bH_R}^2 = \Op{ \frac{1}{\min \braces{p, qT}} }, \quad \frac{1}{q}\norm{\hat \bC - \bC \bH_C}^2 = \Op{\frac{1}{\min \braces{q, pT}}}.\]
\end{proof}


\subsection{Asymptotic behavior of \texorpdfstring{$\bV_{R, pqT}$, $\bV_{C, pqT}$, ${\hbR^\top \bR }/{p}$,  ${\hbC^\top \bC }/{q}$, $\bH_C$ and $\bH_R$}{V, H, hat R top R/p and hat C top C/q}} \label{sec:proof Rhat R}


In this section, we study the asymptotic behavior of $\bV_{R, pqT}$, $\bV_{C, pqT}$, ${\hbR^\top \bR }/{p}$,  ${\hbC^\top \bC }/{q}$, $\bH_C$ and $\bH_R$.
The main results of this section include Proposition \ref{thm:bound V} on the convergence of $\bV_{R, pqT}$ and $\bV_{C, pqT}$, Proposition \ref{thm:bound H} on the convergence of $\bH_C$ and $\bH_R$, and Proposition \ref{prop:RhatR} on the convergence of  ${\hbR^\top \bR }/{p}$ and  ${\hbC^\top \bC }/{q}$.

\begin{proposition} \label{thm:bound V}
    Under Assumption \ref{assume:alpha-mixing}-\ref{assume:eigen-val}, we have, as $p, q, T \rightarrow \infty$:
    \begin{eqnarray}
        \bV_{R, pqT} & = & \frac{1}{p} \hbR^\top \left( \frac{1}{pqT} \sum_{t=1}^{T}  \bY_t \bY_t^\top \right) \hbR \nonumber \\
        & = & \frac{1}{p} \hbR^\top \bR \left( \frac{1}{q T} \sum_{t=1}^{T} \bF_t \bC^\top \bC \bF_t^\top \right) \frac{1}{p}  \bR^\top \hbR + \op{1} \nonumber \\
        & \convprob & \bV_R, \nonumber \\
        \bV_{C, pqT} & = & \frac{1}{p} \hbC^\top \left( \frac{1}{pqT} \sum_{t=1}^{T} \bY_t^\top \bY_t  \right) \hbC \nonumber \\
        & = & \frac{1}{p} \hbC^\top \bC \left( \frac{1}{T} \sum_{t=1}^{qT} \bF_t^\top \bR^\top \bR \bF_t \right) \frac{1}{p}  \bC^\top \hbC + \op{1} \nonumber \\
        &  \convprob & \bV_C, \nonumber
    \end{eqnarray}
    $\norm{\bV_{R, pqT}}_2 = \Op{1}$ and $\norm{\bV_{R, pqT}^{-1}}_2 = \Op{1}$,
    where $\bV_R$ is the diagonal matrix consisting of the eigenvalues of $\bSigma_{FC}^{1/2} \; \bOmega_R \; \bSigma_{FC}^{1/2}$ and $\bV_C$ is the diagonal matrix consisting of the eigenvalues of $\bSigma_{FR}^{1/2} \; \bOmega_C \; \bSigma_{FR}^{1/2}$.
    Covariance $\bSigma_{FC} = \E{\bF_t \frac{{\bC}^\top \bC}{q} \bF_t^\top}$, $\bSigma_{FR} = \E{\bF_t^\top \frac{{\bR}^\top \bR}{p} \bF_t}$.
    Matrices $\bOmega_R$ and $\bOmega_C$ are defined in Assumption \ref{assume:loading_matrix}.
\end{proposition}

\begin{proof}
    From $\frac{1}{p q T} \sum_{t=1}^{T} \bY_t \bY_t^\top \hbR = \hbR \bV_{R, pqT}$ and $\frac{1}{p} \hbR^\top \hbR = \bI_k$, we have
    \[
    \bV_{R, pqT} = \frac{1}{p} \hbR^\top \left( \frac{1}{pqT} \sum_{t=1}^{T} \bY_t^\top \bY_t  \right) \hbR
    \]
    $\bV_{R, pqT}$ is the $k \times k$ diagonal matrix of the first $k$ largest eigenvalues of $\hbM_R \defeq \frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top$ in decreasing order. By definition of $\hbM_R$, we have
    \begin{eqnarray}
        \hbM_R & = &  \frac{1}{p q T} \bR \sum_{t = 1}^{T} \bF_t \bC^\top \bC \bF_t^\top \bR^\top + \frac{1}{p q T} \sum_{t=1}^{T} \bR  \bF_t \bC^\top \bE_t^\top  + \frac{1}{p q T} \sum_{t=1}^{T} \bE_t \bC \bF_t^\top \bR^\top + \frac{1}{p q T} \sum_{t=1}^{T} \bE_t \bE_t^\top \nonumber
    \end{eqnarray}
    Applying Lemma \ref{thm:lemma-3terms}, we have
    \begin{eqnarray}
        \norm{\frac{1}{p q T} \sum_{t=1}^{T} \bR  \bF_t \bC^\top \bE_t^\top}  & \le & \frac{1}{p q T} \norm{\bR} \norm{\sum_{t=1}^{T}  \bF_t \bC^\top \bE_t^\top}_F = \Op{ \frac{1}{\sqrt{q T}} }, \nonumber \\
        \norm{ \frac{1}{p q T} \sum_{t=1}^{T} \bE_t \bC \bF_t^\top \bR^\top} & \le &  \frac{1}{p q T} \norm{\bR} \norm{\sum_{t=1}^{T} \bE_t \bC \bF_t^\top}_F = \Op{ \frac{1}{\sqrt{q T}} }, \nonumber \\
        \norm{ \frac{1}{p q T} \sum_{t=1}^{T} \bE_t \bE_t^\top } & \le & \frac{1}{p q T} \norm{  \sum_{t=1}^{T} \bE_t \bE_t^\top }_F = \Op{ \frac{1}{\sqrt{p}} + \frac{1}{\sqrt{q T}} }.  \nonumber
    \end{eqnarray}
    Then,
    \begin{eqnarray}
        \norm{ \hbM_R - \frac{1}{p q T} \bR \sum_{t = 1}^{T} \bF_t \bC^\top \bC \bF_t^\top \bR^\top } & = & \Op{\frac{1}{\delta_{pqT}}}, \nonumber
    \end{eqnarray}
    where $\delta_{pqT} = 1 / \min \braces{\sqrt{p}, \sqrt{qT}}$.
    We also have
    \begin{equation*}
        \begin{aligned}
            & \norm{\frac{1}{p q T} \bR \sum_{t = 1}^{T} \bF_t \bC^\top \bC \bF_t^\top \bR^\top - \E{ \frac{1}{p q T} \bR \sum_{t = 1}^{T} \bF_t \bC^\top \bC \bF_t^\top \bR^\top }} \\
            & \le \norm{\frac{1}{T} \sum_{t = 1}^{T}  \paran{\bF_t (\bC^\top \bC/q) \bF_t^\top - \E{ \bF_t (\bC^\top \bC/q) \bF_t^\top} } } \cdot \norm{\bR}^2/p\\
            & = \Op{ \frac{1}{\sqrt{T}} }.
        \end{aligned}
    \end{equation*}

    Together, we have
    \[
    \norm{ \hbM_R - \E{ \frac{1}{p q T} \bR \sum_{t = 1}^{T} \bF_t \bC^\top \bC \bF_t^\top \bR^\top }} = \op{1}.
    \]
    Using the inequality that for the $i$-th eigenvalue, $\abs{\lambda_i \paran{\hbA} - \lambda_i \paran{\bA}} \le \norm{\hbA - \bA}_2$, we have
    \[
    \abs{V_{R, pqT, i} - V_{R, i}} = \op{1}, \quad \text{for } 1 \le i \le k,
    \]
    and $\bV_{R, pqT}  \convprob \bV_R$.
    % Hence, it suffices to prove that the first $k$ eigenvalues of $\frac{1}{p q T} \bR \sum_{t = 1}^{T} \bF_t \bC^\top \bC \bF_t^\top \bR^\top$
    Further we have the first $k$ eigenvalues of $\frac{1}{p q T} \bR \sum_{t = 1}^{T} \bF_t \bC^\top \bC \bF_t^\top \bR^\top$ are bounded away from both zero and infinity.
    Thus, $\norm{\bV_{R, pqT}}_2 = \Op{1}$ and $\norm{\bV_{R, pqT}^{-1}}_2 = \Op{1}$.
    Results for $\bV_{C, pqT}$ are obtained in a similar fashion.
\end{proof}

\begin{proposition}  \label{thm:bound H}
    Under Assumption \ref{assume:alpha-mixing}-\ref{assume:eigen-val}, we have
    \[
    \norm{\bH_R} = \Op{1}, \quad \text{and} \quad \norm{\bH_C} = \Op{1}.
    \]
\end{proposition}

\begin{proof}
    Applying results from Proposition \ref{thm:bound V} and Lemma \ref{thm:lemma-3terms}, we obtain
    \begin{equation*}
        \begin{aligned}
            \norm{\bH_R} = \norm{\frac{1}{p q T} \sum_{t=1}^{T} \bF_t \bC^\top \bC \bF_t^\top \bR^\top \hbR \bV_{R, pqT}^{-1}}
            \le \norm{\frac{1}{T} \sum_{t=1}^{T} \bF_t (\bC^\top \bC/q) \bF_t^\top} \norm{\bR}\norm{\hbR}/p \norm{\bV_{R, pqT}^{-1}}
            = \Op{1},  \\
            \norm{\bH_C} = \norm{\frac{1}{p q T} \sum_{t=1}^{T} \bF_t^\top \bR^\top \bR \bF_t \bC^\top \hbC \bV_{C, pqT}^{-1}}
            \le  \norm{\frac{1}{T} \sum_{t=1}^{T} \bF_t^\top (\bR^\top \bR/p) \bF_t} \norm{\bC} \norm{\hbC} / q  \norm{\bV_{C, pqT}^{-1}}
            = \Op{1}.
        \end{aligned}
    \end{equation*}
\end{proof}


\begin{lemma} \label{lemma:I-II-II}
    Under Assumption \ref{assume:alpha-mixing} - \ref{assume:CLT}, we have
    \begin{enumerate}[label=(\alph*) ]
        \item  $\frac{1}{p q T} \sum_{t=1}^{T} \hbR^\top \bE_t \bC \bF_t^\top \bR_{i \cdot} = \Op{\frac{1}{\delta_{pqT} \sqrt{q T}}}$,
        \item  $\frac{1}{p q T} \sum_{t=1}^{T} \hbR^\top \bR \bF_t \bC^\top \be_{t, i \cdot} = \Op{\frac{1}{\sqrt{q T }} }$
        \item $\frac{1}{p q T} \sum_{t=1}^{T} \hbR^\top \bE_t \be_{t, i \cdot} = \Op{\frac{1}{\delta_{pqT} \sqrt{q T}}} + \Op{ \frac{1}{\delta_{pqT} \sqrt{p}}}$
    \end{enumerate}
\end{lemma}

\begin{proof}
    \begin{enumerate}[label=(\alph*) ]
        \item \begin{eqnarray}
            {\rm I} & = & \frac{1}{p q T} \sum_{t=1}^{T} \hbR^\top \bE_t \bC \bF_t^\top \bR_{i \cdot} = \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q}  \hbR_{l \cdot} e_{t, lj} \bC_{j \cdot}^\top \bF_t^\top \bR_{i \cdot} \nonumber \\
            & = & \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} ( \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} ) e_{t, lj} \bC_{j \cdot}^\top \bF_t^\top \bR_{i \cdot} + \bH_R^\top \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \bR_{l \cdot} e_{t, lj} \bC_{j \cdot}^\top \bF_t^\top \bR_{i \cdot} \nonumber \\
            & = & {\rm I_1} + {\rm I_2}.  \nonumber % // & = & = \Op{\frac{1}{\delta_{pqT} \sqrt{q T}}}. \nonumber
        \end{eqnarray}
        We bound each term as follows.
        \begin{eqnarray}
            \norm{\rm I_1} & = & \norm{\frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} ( \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} )\bC_{j \cdot}^\top  e_{t, lj} \bF_t^\top \bR_{i \cdot}} \nonumber \\
            & \le & \frac{1}{\sqrt{q T}}  \left( \frac{1}{p} \sum_{l=1}^{p} \norm{\hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} }^2 \right)^{1/2} \left( \frac{1}{p} \sum_{l=1}^{p} \norm{ \frac{1}{ \sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} e_{t, lj} \bC_{j \cdot}^\top \bF_t^\top }^2 \right)^{1/2} \norm{\bR_{i \cdot}}  \nonumber \\
            & = & \frac{1}{\sqrt{q T}}  \cdot \Op{\frac{1}{\delta_{pqT}}} \cdot \Op{1}, \nonumber
        \end{eqnarray}
        where the last equality results from Theorem \ref{thm:Rhat_F_norm_convg} and Lemma \ref{assume:factor_noise_weak_corr_0}.
        We also have
        \begin{eqnarray}
            \norm{\rm I_2} & = & \frac{1}{\sqrt{p q T}} \norm{ \bH_R^\top \left( \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \bR_{l \cdot} e_{t, lj} \bC_{j \cdot}^\top \bF_t^\top \right) \bR_{i \cdot}} = \Op{\frac{1}{\sqrt{p q T}}}, \nonumber
        \end{eqnarray}
        where the last equality results from by Markov Theorem, Lemma \ref{assume:moments_0} (b) and Proposition \ref{thm:bound H}.
        %\textcolor{red}{Double checked. Right!}
        \item \begin{eqnarray}
            {\rm II} & = & \frac{1}{p q T} \sum_{t=1}^{T} \hbR^\top \bR \bF_t \bC^\top \be_{t, i \cdot} = \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \hbR_{l \cdot} \bR_{l \cdot}^\top \bF_t \sum_{j=1}^{q} \bC_{j \cdot} e_{t, ij} \nonumber \\
            & = &  \frac{1}{p q T} \sum_{l=1}^{p} \left( \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} \right) \bR_{l \cdot}^\top \sum_{t=1}^{T} \sum_{j=1}^{q} \bF_t \bC_{j \cdot} e_{t, ij} + \frac{1}{p q T} \sum_{l=1}^{p} \bH_R^\top \bR_{l \cdot} \bR_{l \cdot}^\top \sum_{t=1}^{T} \sum_{j=1}^{q}  \bF_t \bC_{j \cdot} e_{t, ij} \nonumber  \\
            & = & {\rm II}_1 + {\rm II}_2. \nonumber % \\ & = & \Op{\frac{1}{\sqrt{q T }} }. \nonumber
        \end{eqnarray}
        We bound each term as follows.
        \begin{eqnarray}
            \norm{{\rm II}_1} & = & \norm{\frac{1}{p q T} \sum_{l=1}^{p} \left( \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} \right) \bR_{l \cdot}^\top \sum_{t=1}^{T} \sum_{j=1}^{q} \bF_t \bC_{j \cdot} e_{t, ij} }  \nonumber \\
            & \le & \frac{1}{\sqrt{q T }} \left( \frac{1}{p}\sum_{l=1}^{p} \norm{\hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot}}^2 \right)^{1/2} \left( \frac{1}{p}\sum_{l=1}^{p} \norm{ \bR_{l \cdot}^\top \frac{1}{\sqrt{q T }} \sum_{t=1}^{T} \sum_{j=1}^{q} \bF_t \bC_{j \cdot} e_{t, ij}}^2 \right)^{1/2} \nonumber \\
            & \le & \frac{1}{\sqrt{q T }} \left( \frac{1}{p}\sum_{l=1}^{p} \norm{\hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot}}^2 \right)^{1/2} \left( \frac{1}{p}\sum_{l=1}^{p} \norm{ \bR_{l \cdot} }^2 \cdot \norm{\frac{1}{\sqrt{q T }} \sum_{t=1}^{T} \sum_{j=1}^{q} \bF_t \bC_{j \cdot} e_{t, ij}}^2 \right)^{1/2} \nonumber \\
            & = & \Op{\frac{1}{ \delta_{pqT} \sqrt{q T }} } \qquad \text{ by Theorem \ref{thm:Rhat_F_norm_convg} and Lemma \ref{assume:factor_noise_weak_corr_0}. }  \nonumber
        \end{eqnarray}
        Similarly,
        \begin{equation*}
            \begin{aligned}
                \norm{{\rm II}_2} & =  \norm{\frac{1}{p q T} \sum_{l=1}^{p} \bH_R^\top \bR_{l \cdot} \bR_{l \cdot}^\top \sum_{t=1}^{T} \sum_{j=1}^{q}  \bF_t \bC_{j \cdot} e_{t, ij}}
                 =  \frac{1}{\sqrt{q T }}  \norm{\frac{1}{p} \sum_{l=1}^{p} \bH_R^\top \bR_{l \cdot} \bR_{l \cdot}^\top} \cdot \norm{ \frac{1}{\sqrt{q T }} \sum_{t=1}^{T} \sum_{j=1}^{q}  \bF_t \bC_{j \cdot} e_{t, ij}} \\
                & =  \Op{\frac{1}{\sqrt{q T }} }.
            \end{aligned}
        \end{equation*}
        Combing all the terms, we have
        \[
        \norm{{\rm II}} = \Op{\frac{1}{\sqrt{q T }} }.
        \]
        \item \begin{eqnarray}
            {\rm III} & = & \frac{1}{p q T} \sum_{t=1}^{T} \hbR^\top \bE_t \be_{t, i \cdot} =  \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \hbR_{l \cdot} \be_{t, l \cdot}^\top \be_{t, i \cdot} = \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \hbR_{l \cdot} e_{t, lj} e_{t, ij} \nonumber \\
            & = & \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} \right) e_{t, lj} e_{t, ij} +  \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \bH_R^\top \bR_{l \cdot} e_{t, lj} e_{t, ij} \nonumber \\
            & = & \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} \right) \left( e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} \right) \nonumber \\
            & & + \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} \right) \E{e_{t, lj} e_{t, ij}} \nonumber \\
            & & + \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \bH_R^\top \bR_{l \cdot} \left( e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} \right)  \nonumber \\
            & & +  \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \bH_R^\top \bR_{l \cdot} \E{e_{t, lj} e_{t, ij}} \nonumber \\
            & = & {\rm III}_1 + {\rm III}_2 + {\rm III}_3 + {\rm III}_4 \nonumber %  \\ & = & \Op{\frac{1}{\delta_{pqT} \sqrt{q T}}} + \Op{ \frac{1}{\delta_{pqT} \sqrt{p}}} \nonumber
        \end{eqnarray}
        We bound each term as follows.
        \begin{eqnarray}
            \norm{ \rm III_1 } &  = & \norm{ \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} \right) \left( e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} \right)} \nonumber \\
            & \le & \frac{1}{\sqrt{q T}} \left( \frac{1}{p} \sum_{l=1}^{p} \norm{ \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} }^2 \right)^{1/2} \cdot \left( \frac{1}{p} \sum_{l=1}^{p} \paran{ \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \left( e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} \right) }^2 \right)^{1/2} \nonumber \\
            & = & \Op{\frac{1}{\delta_{pqT} \sqrt{q T}}} \qquad \text{by Lemma \ref{assume:moments_Et_0} and Markov inequality.} \nonumber
        \end{eqnarray}
        \begin{eqnarray}
            \norm{\rm III_2} & = &\norm{ \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} \right) \E{e_{t, lj} e_{t, ij}} } \nonumber \\
            & \le & \frac{1}{\sqrt{p}} \left( \frac{1}{p} \sum_{l=1}^{p} \norm{ \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} }^2 \right)^{1/2} \cdot \left( \frac{1}{p}  \sum_{l=1}^{p} \left( \frac{1}{q T} \sum_{t=1}^{T} \sum_{j=1}^{q} \E{e_{t, lj} e_{t, ij}} \right)^2 \right)^{1/2} \nonumber \\
            & = & \Op{ \frac{1}{\delta_{pqT} \sqrt{p}}} \qquad \text{ by Lemma \ref{assume:cross_row_col_corr_0}.} \nonumber
        \end{eqnarray}

        \begin{eqnarray}
            \norm{\rm III_3} & \le &\norm{ \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q}  \bR_{l \cdot} \left( e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} \right)} \cdot \norm{\bH_R} \nonumber \\
            & = & \Op{\frac{1}{\sqrt{p q T}}} \nonumber \quad  \text{by Lemma \ref{assume:moments_0} (a) and Proposition \ref{thm:bound H}. }
        \end{eqnarray}
        \begin{eqnarray}
            \norm{\rm III_4} & = & \norm{ \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} \bH_R^\top \bR_{l \cdot} \E{e_{t, lj} e_{t, ij}} } \nonumber \\
            & \le &  \frac{1}{p}
            \cdot \norm{\bH_R^\top}
            \cdot \sum_{l=1}^{p} \left| \frac{1}{q T} \sum_{t=1}^{T} \sum_{j=1}^{q} \E{e_{t, lj} e_{t, ij}} \right| \cdot \max_{l\in[p]} {\norm{\bR_{l \cdot}} } \nonumber \\
            & = & \bigO{\frac{1}{p}} \nonumber \qquad \text{ by Assumption \ref{assume:loading_matrix} and Lemma \ref{assume:cross_row_col_corr_0}.}
        \end{eqnarray}
        Combing the result on each term, we obtain
        %\noindent\textbf{Term III}
        \[ \norm{\rm III} = \Op{\frac{1}{\delta_{pqT} \sqrt{q T}}} + \Op{ \frac{1}{\delta_{pqT} \sqrt{p}}}. \]
    \end{enumerate}
\end{proof}

In the following analysis, we use the fact that for positive definite matrices $\bA$ and $\bB$, the eigenvalues of $\bA \bB$, $\bB \bA$ and $\bA^{1/2} \bB \bA^{1/2}$ are the same.

\begin{proposition}  \label{prop:RhatR}
Under Assumption \ref{assume:alpha-mixing}-\ref{assume:eigen-val},
\[
\underset{p, q, T \rightarrow \infty}{\rm plim}\frac{\hat \bR^\top \bR }{p} = \bQ_R, \quad \text{and} \quad \underset{p, q, T \rightarrow \infty}{\rm plim}\frac{\hat \bC^\top \bC }{q} = \bQ_C.
\]
The matrix $\bQ_R \in \RR^{k \times k}$ and $\bQ_C \in \RR^{r \times r}$ are given, respectively, by
\[
\bQ_R = \bV_R^{1/2} \; \bPsi_R^\top \; \bSigma_{FC}^{- 1/2} \quad \text{and} \quad \bQ_C = \bV_C^{1/2} \; \bPsi_C^\top \; \bSigma_{FR}^{- 1/2},
\]
where $\bSigma_{FC} = \E{\bF_t \frac{{\bC}^\top \bC}{q} \bF_t^\top}$, $\bSigma_{FR} = \E{\bF_t^\top \frac{{\bR}^\top \bR}{p} \bF_t}$, $\bV_R$ ($\bV_C$) is a diagonal matrix with diagonal entries being the the eigenvalues of $\bSigma_{FC}^{1/2} \; \bOmega_{R} \; \bSigma_{FC}^{1/2}$ ($\bSigma_{FR}^{1/2} \; \bOmega_{C} \; \bSigma_{FR}^{1/2}$) in decreasing order, $\bPsi_R$ ($\bPsi_C$) is the corresponding eigenvector matrix such that $\bPsi_R^\top \bPsi_R = \bI$ ($\bPsi_C^\top \bPsi_C = \bI$), and $\bOmega_{R}$ ($\bOmega_{C}$) is defined in Lemma \ref{assume:loading_matrix}.
\end{proposition}
%\noindent\textbf{Proof of Proposition \ref{prop:RhatR}}
\begin{proof}
Let $\bX_t = \bF_t \bC^\top$, multiply the identify $\frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top \hbR = \hbR \bV_{R, pqT}$ on both sides by $\frac{1}{p}  \left( \frac{1}{qT} \sum_{t=1}^{T} \bX_t \bX_t^\top \right)^{1/2} \bR^\top$ to obtain:
\[
\frac{1}{p}  \left( \frac{1}{qT} \sum_{t=1}^{T} \bX_t \bX_t^\top \right)^{1/2} \bR^\top \frac{1}{p q T} \sum_{t = 1}^{T} \bY_t \bY_t^\top \hbR =  \left( \frac{1}{qT} \sum_{t=1}^{T} \bX_t \bX_t^\top \right)^{1/2} \frac{\bR^\top \hbR}{p} \bV_{R, pqT}.
\]
Expanding $\bY_t \bY_t^\top$ with $\bY_t = \bR \bF_t \bC^\top + \bE_t$, we can rewrite the above as
\begin{equation} \label{eqn:lemma-decomp}
 \left( \frac{1}{qT} \sum_{t=1}^{T} \bX_t \bX_t^\top \right)^{1/2} \frac{\bR^\top \hbR}{p} \bV_{R, pqT}
 =  \left( \frac{1}{qT} \sum_{t=1}^{T} \bX_t \bX_t^\top \right)^{1/2}  \frac{\bR^\top \bR}{p}  \left( \frac{1}{qT} \sum_{t=1}^{T} \bX_t \bX_t^\top \right) \frac{\bR^\top \hbR}{p} + d_{p q T},
 \end{equation}
where
\begin{equation*}
    \begin{aligned}
        d_{pqT}
        =   \left( \frac{1}{qT} \sum_{t=1}^{T} \bX_t \bX_t^\top \right)^{1/2}
        \left[ \frac{\bR^\top \bR}{p} \cdot \frac{1}{pqT} \sum_{t=1}^{T} \bF_t \bC^\top \bE_t^\top \hbR
        + \frac{1}{p^2qT} \sum_{t=1}^{T} \bR^\top \bE_t \bC \bF_t^\top \bR^\top \hbR
        + \frac{1}{p^2 qT} \sum_{t=1}^{T}  \bR^\top \bE_t \bE_t^\top \hbR  \right].
    \end{aligned}
\end{equation*}
We have
\begin{equation*}
    \begin{aligned}
        \frac{1}{qT} \sum_{t=1}^{T} \bX_t \bX_t^\top & = \frac{1}{T} \sum_{t=1}^{T} \bF_t (\bC^\top\bC/q) \bF_t^\top \\
        & = \frac{1}{T} \sum_{t=1}^{T} \paran{\bF_t (\bC^\top\bC/q) \bF_t^\top - \E{\bF_t (\bC^\top\bC/q) \bF_t^\top} } + \frac{1}{T} \sum_{t=1}^{T} \E{\bF_t (\bC^\top\bC/q) \bF_t^\top} \\
        & = \Op{1}.
    \end{aligned}
\end{equation*}
Proof of Lemma \ref{lemma:I-II-II} (a) shows that $\frac{1}{pqT} \sum_{t=1}^{T} \bF_t \bC^\top \bE_t^\top \hbR = \op{1}$.
Using Lemma \ref{lemma:I-II-II} (b), we have
\begin{equation*}
    \begin{aligned}
       \norm{ \frac{1}{p^2qT}  \sum_{t=1}^{T} \hbR^{\top} \bR \bF_t \bC^\top \bE_t^\top \bR }
       & =  \norm{ \frac{1}{p^2qT} \sum_{i=1}^p  \sum_{t=1}^{T}   \hbR^{\top} \bR \bF_t \bC^\top \be_{t,i\cdot}^\top \bR_{i\cdot} } \\
       & \le \paran{ \frac{1}{p} \sum_{i=1}^p  \norm{\frac{1}{pqT} \sum_{t=1}^{T}   \hbR^{\top} \bR \bF_t \bC^\top \be_{t,i\cdot}^\top}^2 }^{1/2} \paran{ \frac{1}{p} \sum_{i=1}^p \norm{\bR_{i\cdot}} }^{1/2} \\
       & = \op{1}.
    \end{aligned}
\end{equation*}
Using Lemma \ref{lemma:I-II-II} (c) in the same way as above, we have $\frac{1}{p^2 qT} \sum_{t=1}^{T}  \bR^\top \bE_t \bE_t^\top \hbR  = \op{1}$.
Putting all together, we have $d_{pqT}  = \op{1}$.

Define
\begin{eqnarray}
\bA_{pqT} & = &  \left( \frac{1}{qT} \sum_{t=1}^{T} \bX_t \bX_t^\top \right)^{1/2} \frac{\bR^\top \bR}{p}  \left( \frac{1}{qT} \sum_{t=1}^{T} \bX_t \bX_t^\top \right)^{1/2},  \nonumber \\
\bB_{pqT} & = &   \left( \frac{1}{qT} \sum_{t=1}^{T} \bX_t \bX_t^\top \right)^{1/2} \frac{\bR^\top \hbR}{p}, \nonumber
\end{eqnarray}
we rewrite equation (\ref{eqn:lemma-decomp}) as
\begin{equation}
\bB_{pqT} \bV_{R, pqT} = \left( \bA_{pqT} + d_{p q T} \bB_{pqT}^{-1} \right) \bB_{pqT}. \nonumber
\end{equation}
Each column of $\bB_{pqT}$ is an eigenvector of the matrix $\left( \bA_{pqT} + d_{p q T} \bB_{pqT}^{-1} \right)$

By Proposition \ref{thm:bound V}, we have
\begin{equation} \label{eqn:BtB}
    \begin{aligned}
        \bB_{pqT}^\top \bB_{pqT} & = \frac{\hbR^\top \bR}{p}  \left( \frac{1}{qT} \sum_{t=1}^{T} \bF_t (\bC^\top\bC/q) \bF_t^\top \right) \frac{\bR^\top \hbR}{p}  \convprob \bV_R,
    \end{aligned}
\end{equation}
and $\bV_R$  is the diagonal matrix consisting of the eigenvalues of $\bSigma_{FC}^{1/2} \; \bOmega_{R} \; \bSigma_{FC}^{1/2}$.
Thus the eigenvalues of $\bB_{pqT}^\top \bB_{pqT}$ are asymptotically bounded away from infinity and zero, and $ \bB_{pqT}^{-1} = \Op{1}$.

Let $\bV_{R, pqT}^*$ be a diagonal matrix consisting of the diagonal elements of $\bB_{pqT}^\top \bB_{pqT}$.
From \eqref{eqn:BtB}, we have
\begin{equation} \label{eqn:V-star-conv}
    \bV_{R, pqT}^* \convprob \bV_R.
\end{equation}
Denote
\begin{equation} \label{eqn:psi-r-pqt}
    \bPsi_{R, pqT} = \bB_{pqT} {\bV_{R, pqT}^*}^{-1/2},
\end{equation}
then $\norm{\bPsi_{R, pqT}} = 1$ and
\begin{equation}
\bPsi_{R, pqT} \bV_{R, pqT} = \left( \bA_{pqT} + d_{p q T} \bB_{pqT}^{-1} \right) \bPsi_{R, pqT}, \nonumber
\end{equation}
that is, each column of $\bPsi_{R, pqT}$ is an eigenvector of $\bA_{pqT} + d_{pqT} \bB_{pqT}^{-1}$.

From Lemma \ref{assume:factor-noise-matrix} and \ref{assume:loading_matrix}, $d_{pqT} = \op{1}$, and $ \bB_{pqT}^{-1}  = \Op{1}$, we have $\bA_{pqT} \stackrel{p}{\longrightarrow}  \bSigma_{FC}^{1/2} \; \bOmega_{R} \; \bSigma_{FC}^{1/2}$ and $d_{pqT} \bB_{pqT}^{-1} =  \op{1}$.
By eigenvector perturbation theory \citep{franklin2012matrix} and Assumption \ref{assume:eigen-val}, there exists a unique eigenvector matrix $\bPsi_R$ of $\bSigma_{FC}^{1/2} \; \bOmega_{R} \; \bSigma_{FC}^{1/2}$ such that $\norm{\bPsi_{R, pqT} - \bPsi_R } = \op{1}$, where $\bPsi_R$ is the eigenvector matrix of $\bSigma_{FC}^{1/2} \; \bOmega_{R} \; \bSigma_{FC}^{1/2}$.

From \eqref{eqn:psi-r-pqt} and \eqref{eqn:V-star-conv}, we have
\[
\frac{\bR^\top \hbR}{p}  = \left( \frac{1}{qT} \sum_{t=1}^{qT} \bX_t \bX_t^\top \right)^{- 1/2} \bPsi_{R, pqT} {\bV_{R, pqT}^*}^{1/2} \; \stackrel{p}{\longrightarrow} \; \bSigma_{FC}^{- 1/2} \; \bPsi_R \; \bV_R^{1/2}.
\]
\end{proof}



\subsection{Theorem \ref{thm:asymp normality of R/C}: Asymptotic distribution of \texorpdfstring{$\hbR_{i \cdot} - \bH_R^\top \bR_{i \cdot}$}{estimation errors of R}} \label{sec:proof for R}

We make use of the following equality for each row of equation (\ref{eqn:proof:hatR-RH}): for each row vector $\bR_{i \cdot} \in \mathbb{R}^{k}$, $i \in [p]$, we have
\begin{eqnarray} \label{eqn:proof:hatR-RH-row}
\hbR_{i \cdot} - \bH_R^\top \bR_{i \cdot} & = & \bV_{R, pqT}^{-1} \left( \frac{1}{p q T} \sum_{t=1}^{T} \hbR^\top \bE_t \bC \bF_t^\top \bR_{i \cdot} + \frac{1}{p q T} \sum_{t=1}^{T} \hbR^\top \bR \bF_t \bC^\top \be_{t, i \cdot} + \frac{1}{p q T} \sum_{t=1}^{T} \hbR^\top \bE_t \be_{t, i \cdot} \right) \nonumber \\
& = & \bV_{R, pqT}^{-1} \left( {\rm I} + {\rm II} + {\rm III} \right).
\end{eqnarray}
In the following proofs, we let $\delta_{pqT} = \min \braces{\sqrt{p}, \sqrt{qT}}$ and $\gamma_{pqT} = \min \braces{ \sqrt{q}, \sqrt{pT}}$.
% The following Lemma \ref{lemma:I-II-II} gives convergence rate for each term in (\ref{eqn:proof:hatR-RH-row}).


\paragraph{Proof of Theorem \ref{thm:asymp normality of R/C}}
\begin{proof}
The dominant terms in equation (\ref{eqn:proof:hatR-RH-row}) are ${\rm II}_2 + {\rm III}_2 = \Op{\frac{1}{\sqrt{qT}}} + \Op{\frac{1}{p}}$.

If $\sqrt{q T} / p \rightarrow 0$, the dominant term in equation (\ref{eqn:proof:hatR-RH-row}) is ${\rm II}$. Then
\begin{eqnarray}
\sqrt{qT} \left( \hbR_{i \cdot} - \bH_R^\top \bR_{i \cdot} \right) & = & \bV_{R, pqT}^{-1} \frac{\hbR^\top \bR }{p} \frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \bF_t \bC^\top \be_{t, i \cdot} + \op{1} \nonumber \\
& = & \bV_{R, pqT}^{-1} \frac{\hbR^\top \bR }{p} \frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \bF_t \bC^\top \be_{t, i \cdot} + \op{1} \nonumber \\
&\convdist& \calN\paran{\bzero, \bSigma_{R_i}}, \quad\text{by Lemma \ref{assume:CLT_0} and continuous mapping thoerem.}\nonumber
\end{eqnarray}
where
\begin{equation*}
    \bSigma_{R_i} \defeq \bV_R^{-1}\bQ_R
    \paran{\bPhi_{R,i,11}+\alpha\bPhi_{R,i,12}\bmu_F^\top+\alpha\bmu_F\bPhi_{R,i,21}+\alpha^2\bmu_F\bPhi_{R,i,22}\bmu_F^\top}
    \bQ_R^\top\bV_R^{-1},
\end{equation*}
and $\bPhi_{R,i,\cdot\cdot}$ are given in Theorem \ref{thm:asymp normality of R/C}.
Matrix $\bQ_R \defeq \bV_R^{1/2}\;\bPsi_R^\top\;\tilde\bSigma_{FC}^{- 1/2}$
where $\bV_R$ is a diagonal matrix whose entries are the eigenvalues of $\tilde\bSigma_{FC}^{1/2}\;\bOmega_{R}\;\tilde\bSigma_{FC}^{1/2}$ in decreasing order,  $\bPsi_R$ is the corresponding eigenvector matrix such that $\bPsi_R^\top \bPsi_R = \bI$, $\bOmega_{R}$ defined in Assumption \ref{assume:loading_matrix} and $\tilde\bSigma_{FC}$ is defined in \eqref{eqn:Sigma_FC_FR_tilde}.

If ${\rm lim \, inf} \sqrt{q T} / p \ge \tau > 0$, the dominant term in equation (\ref{eqn:proof:hatR-RH-row}) is ${\rm II_2 + III_2}$. Under certain assumptions,
\begin{eqnarray}
p \left( \hbR_{i \cdot} - \bH_R^\top \bR_{i \cdot} \right) & = & \Op{\frac{p}{\sqrt{q T }} } + \Op{1} = \Op{1}. \nonumber
\end{eqnarray}

Now we consider estimated column loading matrix $\hbC$. Using equation (\ref{eqn:proof:hatC-CH}), we have
\begin{eqnarray} \label{eqn:proof:hatC-CH-row}
\hbC_{j \cdot} - \bH_C^\top \bC_{j \cdot} & = & \bV_{C, pqT}^{-1} \left( \frac{1}{p q T} \sum_{t=1}^{T} \hbC^\top \bE_t^\top \bR \bF_t \bC_{j \cdot} + \frac{1}{p q T} \sum_{t=1}^{T} \hbC^\top \bC \bF_t^\top \bR^\top \be_{t, \cdot j } + \frac{1}{p q T} \sum_{t=1}^{T} \hbC^\top \bE_t^\top \be_{t, \cdot j } \right) \nonumber \\
& = & \bV_{C, pqT}^{-1} \left( {\rm I} + {\rm II} + {\rm III} \right)
\end{eqnarray}

Similar to the proofs of Lemma \ref{lemma:I-II-II}, we have that if $\sqrt{p T} / q \rightarrow 0$, the dominant term in equation (\ref{eqn:proof:hatC-CH-row}) is ${\rm II}$. Then
\begin{eqnarray}
\sqrt{pT} \left( \hbC_{j \cdot} - \bH_C^\top \bC_{j \cdot} \right)
& = & \bV_{C, pqT}^{-1} \frac{\hbC^\top \bC }{q} \frac{1}{\sqrt{pT}} \sum_{t=1}^{T} \bF_t^\top \bR^\top \be_{t, \cdot j } + \op{1} \nonumber \\
&\convdist &\calN\paran{\bzero, \bSigma_{C_j}}, \quad\text{by Lemma \ref{assume:CLT_0} and continuous mapping thoerem.}\nonumber
\end{eqnarray}
where
\begin{equation*}
    \bSigma_{C_j} \defeq \bV_C^{-1}\bQ_C
    \paran{\bPhi_{C,j,11}+\alpha\bPhi_{C,j,12}\bmu_F+\alpha\bmu_F^\top\bPhi_{C,j,21}+\alpha^2\bmu_F^\top\bPhi_{C,j,22}\bmu_F}
    \bQ_C^\top \bV_C^{-1},
\end{equation*}
and $\bPhi_{C,j,\cdot\cdot}$ are Theorem \ref{thm:asymp normality of R/C}.
Matrix $\bQ_C \defeq \bV_C^{1/2}\;\bPsi_C^\top\;\tilde\bSigma_{FR}^{- 1/2}$
where
$\bV_C$ is a diagonal matrix whose entries are the eigenvalues of $\tilde\bSigma_{FR}^{1/2}\;\bOmega_{C}\;\tilde\bSigma_{FR}^{1/2}$ in decreasing order,  $\bPsi_C$ is the corresponding eigenvector matrix such that $\bPsi_C^\top\bPsi_C = \bI$, $\bOmega_{C}$ is defined in Assumption \ref{assume:loading_matrix}, and $\tilde\bSigma_{FR}$ is defined in \eqref{eqn:Sigma_FC_FR_tilde}.

If ${\rm lim \, inf} \sqrt{p T} / q \ge \tau > 0$, then
\begin{eqnarray}
q \left( \hbC_{j \cdot} - \bQ_R^\top \bC_{j \cdot} \right) & = & \Op{\frac{q}{\sqrt{p T }} } + \Op{1} = \Op{1}. \nonumber
\end{eqnarray}
\end{proof}

\subsection{Theorem \ref{thm:asymp_Ft}: Convergence rate of \texorpdfstring{$\hat \bF_t$}{hat F}}  \label{sec:proof F_t}

\paragraph{Proof of Theorem \ref{thm:asymp_Ft}.}
\begin{proof}
Under the assumption that $\frac{1}{p} \hbR^\top \hbR = \bI_{p}$ and $\frac{1}{q} \hbC^\top \hbC = \bI_{q}$,  we have
\[
\hat \bF_t =  \frac{1}{p q} \hbR^\top \bY_t \hbC =  \frac{1}{p q} \hbR^\top \bR \bF_t \bC^\top \hbC + \frac{1}{p q} \hbR^\top \bE_t \hbC.
\]
Writing $\bR = \paran{\bR - \hbR \bH_R^{-1}} + \hbR \bH_R^{-1}$ and
$\bC = \paran{\bC - \hbC \bH_C^{-1}} + \hbC \bH_C^{-1}$, we obtain
\begin{equation} \label{eqn:lemma-Ft-1}
    \begin{aligned}
        \hat \bF_t - \bH_R^{-1} \bF_t {\bH_C^{-1}}^\top
        & = \frac{1}{p q} \hbR^\top \left( \bR - \hbR \bH_R^{-1} \right) \bF_t \left( \bC - \hbC \bH_C^{-1} \right)^\top \hbC \\
        &  + \; \frac{1}{p} \hbR^\top \left( \bR - \hbR \bH_R^{-1} \right) \bF_t {\bH_C^{-1}}^\top  \\
        &  + \; \frac{1}{q} \bH_R^{-1} \bF_t \left( \bC - \hbC \bH_C^{-1} \right)^\top \hbC  \\
        &  + \; \frac{1}{pq} \hbR^\top \bE_t \hbC.
    \end{aligned}
\end{equation}
We further decompose $\hbR = \hbR - \bR \bH_R + \bR \bH_R$ and $\hbC = \hbC - \bC \bH_C + \bC \bH_C$ in the last term of  \eqref{eqn:lemma-Ft-1} and rearrange the equation. We have
\begin{eqnarray} \label{eqn:factor-decomp}
\hat \bF_t - \bH_R^{-1} \bF_t {\bH_C^{-1}}^\top
& = & \frac{1}{p q} \hbR^\top \left( \bR - \hbR \bH_R^{-1} \right) \bF_t \left( \bC - \hbC \bH_C^{-1} \right)^\top \hbC \nonumber \\
&  & + \; \frac{1}{p} \hbR^\top \left( \bR - \hbR \bH_R^{-1} \right) \bF_t {\bH_C^{-1}}^\top \nonumber \\
&  & + \; \frac{1}{q} \bH_R^{-1} \bF_t \left( \bC - \hbC \bH_C^{-1} \right)^\top \hbC \nonumber \\
& & + \; \frac{1}{p q}  \left( \hbR - \bR \bH_R \right)^\top \bE_t \left( \hbC - \bC \bH_C \right) \nonumber \\
& & + \; \frac{1}{p q}  \left( \hbR - \bR \bH_R \right)^\top \bE_t \hbC \nonumber \\
& & + \; \frac{1}{p q} \hbR^\top \bE_t \left( \hbC - \bC \bH_C \right) \nonumber \\
& & + \; \frac{1}{p q} \bH_R^\top \bR^\top \bE_t \bC \bH_C \nonumber \\
& & = \sum_{i=1}^{7} I_i. \nonumber
\end{eqnarray}

Since $\frac{1}{ \sqrt{p} } \norm{\bR - \hbR \bH_R^{-1}} = \op{1}$ and $\frac{1}{ \sqrt{q} } \norm{\bC - \hbC \bH_C^{-1}} = \op{1}$ by Theorem \ref{thm:Rhat_F_norm_convg} and Proposition \ref{thm:bound H}, term $I_1$ is dominated by $I_2$ and $I_3$, and term $I_4$ is dominated by $I_5$ and $I_6$.
Now we bound $I_2$, $I_3$, $I_5$, $I_6$ and $I_7$.
\begin{equation*}
    \begin{aligned}
        I_2
        & = \frac{1}{p} (\hbR - \bR\bH_R)^\top \left( \bR - \hbR \bH_R^{-1} \right) \bF_t {\bH_C^{-1}}^\top
        + \frac{1}{p}  \bH_R^\top \bR^\top \left( \bR - \hbR \bH_R^{-1} \right) \bF_t {\bH_C^{-1}}^\top \\
        & =  \Op{\frac{1}{\delta_{pqT}^2}},
    \end{aligned}
\end{equation*}
by Theorem \ref{thm:Rhat_F_norm_convg} and Proposition \ref{thm:bound H}, and \ref{lemma:F_term_1}.
Similarly, using results in Theorem \ref{thm:Rhat_F_norm_convg}, Proposition \ref{thm:bound H} and Lemma \ref{lemma:F_term_1}, and \ref{lemma:F_term_2}, we have
\[
I_2 = \Op{\frac{1}{\gamma_{pqT}^2}}, \quad I_5 = \Op{\frac{1}{\delta_{pqT}^2}}, \quad I_6 =  \Op{\frac{1}{\gamma_{pqT}^2}}.
\]
Finally, we have
\[
\hat \bF_t - \bH_R^{-1} \bF_t {\bH_C^{-1}}^\top  = \frac{1}{p q} \bH_R^\top \bR^\top \bE_t \bC \bH_C + \Op{\frac{1}{\delta_{pqT}^2}} + \Op{\frac{1}{\gamma_{pqT}^2}} = \Op{\frac{1}{\min \paran{p, q}}},
\]
where we uses results in Lemma \ref{lemma:E_term}.
\end{proof}

\subsubsection{Technical lemmas}

\begin{lemma}  \label{lemma:F_term_1}
	Under Assumption \ref{assume:alpha-mixing}-\ref{assume:eigen-val}, the $k \times k$ matrix
	\[\frac{1}{p} \left( \hbR - \bR \bH_R \right)^\top \bR =  \Op{\frac{1}{\delta_{pqT}^2}}; \]
	The $r \times r$ matrix
	\[\frac{1}{q}  \left( \hbC - \bC \bH_C \right)^\top \bC  = \Op{\frac{1}{\gamma_{pqT}^2}}.\]
\end{lemma}
\begin{proof}
    Using the identity \eqref{eqn:proof:hatR-RH}, we have
    \begin{equation*}
        \begin{aligned}
            \frac{1}{p} \paran{ \hbR - \bR \bH_R }^\top \bR
            & = \bV_{R, pqT}^{-1} \paran{ \frac{1}{p^2 q T} \sum_{t=1}^{T} \hbR^\top \bE_t \bC \bF_t^\top \bR^\top \bR
            + \frac{1}{p^2 q T} \sum_{t=1}^{T} \hbR^\top \bR \bF_t \bC^\top \bE^\top \bR
            + \frac{1}{p^2 q T} \sum_{t=1}^{T} \hbR^\top \bE_t \bE_t^\top \bR } \\
            & = \bV_{R, pqT}^{-1} ({\rm I + II + III}).
        \end{aligned}
    \end{equation*}

    From the following bounds on each term ${\rm I}$, ${\rm II}$, and ${\rm III}$, we get
    \[
    \frac{1}{p} \left( \hbR - \bR \bH_R \right)^\top \bR
    = \Op{\frac{1}{\delta_{pqT} \sqrt{q T}}} + \Op{\frac{1}{\delta_{pqT} \sqrt{p}}} +  \Op{\frac{1}{\sqrt{p q T}}} + \bigO{\frac{1}{p}}
    =  \Op{\frac{1}{\delta^2_{pqT}}}.
    \]

    Similarly, we have
    \[
    \frac{1}{q} \left( \hbC - \bC \bH_C \right)^\top \bC
    = \Op{\frac{1}{\delta_{pqT} \sqrt{p T}}} + \Op{\frac{1}{\delta_{pqT} \sqrt{q}}} +  \Op{\frac{1}{\sqrt{p q T}}} + \bigO{\frac{1}{q}}
    = \Op{\frac{1}{\gamma_{pqT}^2}}.
    \]


    We begin with term I,
    \begin{equation*}
        {\rm I} =
        \frac{1}{p^2 q T} \sum_{t=1}^{T} \paran{\hbR - \bR \bH_R}^\top \bE_t \bC \bF_t^\top \bR^\top \bR
        + \frac{1}{p^2 q T} \sum_{t=1}^{T} \bH_R^\top \bR^\top \bE_t \bC \bF_t^\top \bR^\top \bR = {\rm I_1} + {\rm I_2}
    \end{equation*}
	We have
	\[
	{\rm I} = \Op{\frac{1}{\delta_{pqT} \sqrt{q T}}} + \Op{\frac{1}{\sqrt{p q T}}}.
	\]
	Since,
	\begin{equation*}
        \begin{aligned}
            \norm{ {\rm I_1} } & = \norm{ \frac{1}{p^2 q T} \sum_{t=1}^{T} \paran{\hbR - \bR \bH_R}^\top \bE_t \bC \bF_t^\top \bR^\top \bR }
            \le  \norm{ \frac{1}{p q T} \sum_{t=1}^{T} \sum_{l=1}^{p} \sum_{j=1}^{q} ( \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} )\bC_{j \cdot}^\top  e_{t, lj} \bF_t^\top }
            \cdot \frac{1}{p} \norm{ \bR^\top \bR }  \\
            & \le \frac{1}{\sqrt{q T}}  \left( \frac{1}{p} \sum_{l=1}^{p} \norm{\hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} }^2 \right)^{1/2} \cdot \; \left( \frac{1}{p} \sum_{l=1}^{p} \norm{ \frac{1}{ \sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \bC_{j \cdot}^\top  e_{t, lj} \bF_t^\top }^2 \right)^{1/2}  \cdot  \frac{1}{p} \norm{ \bR^\top \bR }  \\
            & =  \frac{1}{\sqrt{q T}}  \cdot \Op{\frac{1}{\delta_{pqT}}} \cdot \Op{1}  \qquad \text{ using Lemma \ref{assume:factor_noise_weak_corr_0},}  \nonumber
        \end{aligned}
	\end{equation*}
and
	\begin{equation*}
    \begin{aligned}
	\norm{ {\rm I}_2 }
    & = \norm{ \frac{1}{p^2 q T} \sum_{t=1}^{T} \bH_R^\top \bR^\top \bE_t \bC \bF_t^\top \bR^\top \bR }
    \le  \frac{1}{\sqrt{p q T}} \norm{ \bH_R }
    \cdot \norm{ \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \bR^\top \bE_t \bC \bF_t^\top }
    \cdot \frac{1}{p} \norm{\bR^\top \bR} \\
	& = \Op{ \frac{1}{\sqrt{p q T}} }, \qquad \text{ using Lemma \ref{assume:moments_0} and Proposition \ref{thm:bound H}. }
    \end{aligned}
    \end{equation*}

	Second, we deal with term II,
    \begin{equation*}
        {\rm II} = \frac{1}{p^2 q T} \sum_{t=1}^{T} \hbR^\top \bR \bF_t \bC^\top \bE_t^\top \bR
        = \frac{1}{\sqrt{p q T}} \cdot \frac{1}{p} \hbR^\top \bR \cdot  \frac{1}{\sqrt{p q T}} \sum_{t=1}^{T} \bF_t \bC^\top \bE_t^\top \bR = \Op{\frac{1}{\sqrt{p q T }} },
    \end{equation*}
   where we use Proposition \ref{prop:RhatR} and Lemma \ref{assume:moments_0}.

	Finally, we deal with term III,
    \begin{equation*}
        \begin{aligned}
            {\rm III}
            & = \frac{1}{p^2 q T} \sum_{t=1}^{T} \hbR^\top \bE_t \bE_t^\top \bR
            = \frac{1}{p^2 q T} \sum_{t=1}^{T} \paran{\hbR - \bR\bH_R}^\top \bE_t \bE_t^\top \bR
            + \frac{1}{p^2 q T} \sum_{t=1}^{T} \bH_R^\top \bR^\top \bE_t \bE_t^\top \bR \\
            & = \frac{1}{p^2 q T} \sum_{t=1}^{T} \paran{\hbR - \bR\bH_R}^\top \paran{\bE_t \bE_t^\top - \E{\bE_t \bE_t^\top} } \bR
            + \frac{1}{p^2 q T} \sum_{t=1}^{T} \paran{\hbR - \bR\bH_R}^\top  \E{\bE_t \bE_t^\top} \bR \\
            & + \frac{1}{p^2 q T} \sum_{t=1}^{T} \bH_R^\top \bR^\top \paran{\bE_t \bE_t^\top - \E{\bE_t \bE_t^\top} } \bR
            + \frac{1}{p^2 q T} \sum_{t=1}^{T} \bH_R^\top \bR^\top \E{\bE_t \bE_t^\top} \bR \\
            & = {\rm III_1 + III_2 + III_3 + III_4}.
        \end{aligned}
    \end{equation*}

	We have
	\[
	{\rm III} = \Op{\frac{1}{\delta_{pqT} \sqrt{q T}}} + \Op{\frac{1}{\delta_{pqT} \sqrt{p}}} +  \Op{\frac{1}{\sqrt{p q T}}} + \bigO{\frac{1}{p}}
	\]

	Since
	\begin{eqnarray}
	\norm{\rm III_1 }^2
    & = &  \norm{ \frac{1}{p^2 q T} \sum_{t=1}^{T} \paran{\hbR - \bR\bH_R}^\top \paran{\bE_t \bE_t^\top - \E{\bE_t \bE_t^\top} } \bR }^2 \nonumber \\
    &  = & \norm{ \frac{1}{p^2 q T} \sum_{t=1}^{T} \sum_{i=1}^{p} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} \right) \left( e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} \right) \bR_{i \cdot}^\top }^2 \nonumber \\
	& \le & \frac{1}{q T} \frac{1}{p} \sum_{l=1}^{p} \norm{ \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} }^2 \cdot \frac{1}{p} \sum_{l=1}^{p} \norm{ \frac{1}{p} \sum_{i=1}^{p} \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \left( e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} \right) \bR_{i \cdot}^\top }^2 \nonumber \\
    & \le & \frac{1}{q T} \frac{1}{p} \sum_{l=1}^{p} \norm{ \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} }^2
    \cdot \frac{1}{p} \sum_{l=1}^{p}  \frac{1}{p} \sum_{i=1}^{p} \paran{ \frac{1}{\sqrt{q T}} \sum_{t=1}^{T} \sum_{j=1}^{q} \left( e_{t, lj} e_{t, ij} - \E{e_{t, lj} e_{t, ij}} \right) }^2
    \cdot \frac{1}{p} \sum_{i=1}^{p} \norm{\bR_{i \cdot}^\top }^2 \nonumber \\
	& = & \Op{\frac{1}{q T}} \cdot \Op{ \frac{1}{\delta_{pqT}^2}}  \cdot \Op{1}, \nonumber \qquad \text{using Theorem \ref{thm:Rhat_F_norm_convg} and Lemma \ref{assume:moments_Et_0}.}
    \end{eqnarray}
    \begin{eqnarray}
	\norm{\rm III_2}^2
    & = & \norm{\frac{1}{p^2 q T} \sum_{t=1}^{T} \paran{\hbR - \bR\bH_R}^\top  \E{\bE_t \bE_t^\top} \bR}^2  \nonumber \\
    & = &\norm{ \frac{1}{p^2 q T} \sum_{t=1}^{T} \sum_{i=1}^{p} \sum_{l=1}^{p} \sum_{j=1}^{q} \left( \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} \right) \E{e_{t, lj} e_{t, ij}} \bR_{i \cdot}^\top }^2 \nonumber \\
	& \le & \frac{1}{p} \cdot \frac{1}{p} \sum_{l=1}^{p} \norm{ \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} }^2 \cdot \sum_{l=1}^{p} \norm{ \frac{1}{p q T}  \sum_{t=1}^{T} \sum_{i=1}^{p} \sum_{j=1}^{q} \E{e_{t, lj} e_{t, ij}} \bR_{i \cdot}^\top }^2 \nonumber \\
	& \le & \frac{1}{p} \cdot \frac{1}{p} \sum_{l=1}^{p} \norm{ \hbR_{l \cdot} - \bH_R^\top \bR_{l \cdot} }^2
    \cdot \frac{1}{p} \sum_{l=1}^{p} \sum_{i=1}^{p} \paran{ \frac{1}{q T} \sum_{t=1}^{T} \sum_{j=1}^{q} \E{e_{t, lj} e_{t, ij}} }^2
    \cdot \frac{1}{p} \sum_{i=1}^{p} \norm{ \bR_{i \cdot}^\top }^2  \nonumber \\
	& = &  \frac{1}{p} \cdot \Op{ \frac{1}{\delta_{pqT}^2}}  \cdot \bigO{1}  \nonumber \qquad \text{ using Lemma \ref{assume:cross_row_col_corr_0}.} \\
	& = & \Op{ \frac{1}{p \delta_{pqT}^2}}. \nonumber
	\end{eqnarray}
    \begin{equation*}
    \begin{aligned}
	\norm{\rm III_3}
    & = \norm{\frac{1}{p^2 q T} \sum_{t=1}^{T} \bH_R^\top \bR^\top \paran{\bE_t \bE_t^\top - \E{\bE_t \bE_t^\top} } \bR} \\
    & \le \frac{1}{\sqrt{pqT}} \cdot \paran{ \frac{1}{\sqrt{p}}  \norm{\frac{1}{\sqrt{qT}} \sum_{t=1}^{T} \paran{\bE_t \bE_t^\top - \E{\bE_t \bE_t^\top} } } } \cdot \norm{\bH_R} \cdot \frac{1}{p} \norm{ \bR}^2 \\
	& = \Op{\frac{1}{\sqrt{pqT}} },
    \end{aligned}
    \end{equation*}
    \begin{equation*}
        \begin{aligned}
            \norm{\rm III_4}^2
            & = \norm{\frac{1}{p^2 q T} \sum_{t=1}^{T} \bH_R^\top \bR^\top \E{\bE_t \bE_t^\top} \bR }^2
            \le  \frac{1}{p^2} \norm{ \E{\frac{1}{qT} \sum_{t=1}^{T} \bE_t \bE_t^\top } }^2
            \cdot \frac{1}{p^2} \norm{  \bR  }^4
            \cdot \norm{\bH_R}^2 \\
            & = \bigO{\frac{1}{p^2}}, \qquad \text{ by Lemma \ref{assume:cross_row_col_corr_0}.}
        \end{aligned}
	\end{equation*}
\end{proof}

\begin{lemma}  \label{lemma:F_term_2}
	Under Assumption \ref{assume:alpha-mixing} - \ref{assume:CLT},  the $k \times r$ matrix
	\[
    \frac{1}{p q}  \left( \hbR - \bR \bH_R \right)^\top \bE_t \bC =  \Op{\frac{1}{\delta^2_{pqT}}}
    \]
    \[
    \frac{1}{p q} \bR^\top \bE_t \left( \hbC - \bC \bH_C \right) = \Op{\frac{1}{\gamma_{pqT}^2}}
    \]
\end{lemma}

\begin{proof}
Under Assumption \ref{assume:alpha-mixing}-\ref{assume:eigen-val},  we have
\begin{equation} \label{eqn:lemma:F_term_2-1}
    \begin{aligned}
        \frac{1}{pq} \left( \hbR - \bR \bH_R \right)^\top \bE_t \bC  & = \bV_{R, pqT}^{-1^\top} \left(  \frac{1}{p^2 q^2 T} \sum_{s=1}^{T} \hbR^\top \bE_s \bC \bF_s^\top \bR^\top \bE_t \bC \right. \\
        & = + \frac{1}{p^2 q^2 T} \sum_{s=1}^{T} \hbR^\top \bR  \bF_s  \bC^\top \bE_s^\top \bE_t \bC \\
        & \left. + \frac{1}{p^2 q^2 T} \sum_{s=1}^{T} \hbR^\top \bE_s \bE_s^\top \bE_t \bC \right) \\
        & = \bV_{R, pqT}^{-1} ({\rm I + II + III}).
    \end{aligned}
\end{equation}
First, we show that ${\rm I} = \Op{ \frac{1}{\delta_{pqT} \sqrt{q T}} }$ in \eqref{eqn:lemma:F_term_2-1},
\begin{equation*}
    {\rm I} = \frac{1}{p^2 q^2 T} \sum_{s=1}^{T} \hbR^\top \bE_s \bC \bF_s^\top \bR^\top \bE_t \bC
    = \frac{1}{p^2 q^2 T} \sum_{s=1}^{T} \left( \hbR - \bR \bH_R \right)^\top \bE_s \bC \bF_s^\top \bR^\top \bE_t \bC
    + \; \frac{1}{p^2 q^2 T} \sum_{s=1}^{T} \bH_R^\top \bR^\top \bE_s \bC \bF_s^\top \bR^\top \bE_t \bC.
\end{equation*}
For each term on the right hand side, we have
\begin{equation*}
    \begin{aligned}
        \norm{\frac{1}{p^2 q^2 T} \sum_{s=1}^{T} \left( \hbR - \bR \bH_R \right)^\top \bE_s \bC \bF_s^\top \bR^\top \bE_t \bC}
        & \le \frac{1}{\sqrt{pqT}}
        \cdot \frac{1}{\sqrt{p}} \norm{ \hbR - \bR \bH_R }
        \cdot \norm{ \frac{1}{\sqrt{qT}}  \sum_{s=1}^{T} \bE_s \bC \bF_s^\top}_F
        \cdot \norm{ \frac{1}{p q} \bR^\top \bE_t \bC}  \\
        & = \frac{1}{\sqrt{q T}}
        \cdot \frac{1}{\sqrt{p}} \norm{ \hbR - \bR \bH_R }
        \cdot \paran{ \frac{1}{p} \sum_{i=1}^p \norm{ \frac{1}{\sqrt{qT}}  \sum_{s=1}^{T} \sum_{j=1}^q  \bF_s \bC^\top \be_{s,i\cdot}}^2 }^{1/2}
        \cdot \norm{ \frac{1}{p q} \bR^\top \bE_t \bC}  \\
        & = \Op{ \frac{1}{\delta_{pqT} \sqrt{q T}} },
    \end{aligned}
\end{equation*}
where we used Theorem \ref{thm:Rhat_F_norm_convg}, Lemma \ref{assume:factor_noise_weak_corr_0}, Lemma \ref{assume:moments_Et_0} and Markov inequality.
Similarly,
\begin{eqnarray}
\norm{{\rm I_2}} & = & \norm{\frac{1}{p^2 q^2 T} \sum_{s=1}^{T} \bH_R^\top \bR^\top \bE_s \bC \bF_s^\top \bR^\top \bE_t \bC} \nonumber \\
& \le & \frac{1}{\sqrt{pqT}} \norm{\bH_R} \cdot \norm{\frac{1}{\sqrt{pqT}} \sum_{s=1}^{T} \bR^\top \bE_s \bC \bF_s^\top} \cdot \norm{ \frac{1}{pq} \bR^\top \bE_t \bC} \nonumber \\
& = & \Op{ \frac{1}{\sqrt{pqT}} }, \nonumber
\end{eqnarray}
where we used Proposition \ref{thm:bound H}, Lemma \ref{assume:moments_Et_0} and Markov inequality.

Next we consider term ${\rm III}$ in \eqref{eqn:lemma:F_term_2-1}:
\begin{equation}  \label{lemma:F_term_2-2}
    \begin{aligned}
        {\rm III} & = \frac{1}{p^2 q^2 T} \sum_{s=1}^{T} \hbR^\top \bE_s \bE_s^\top \bE_t \bC
        = \frac{1}{p^2 q^2 T} \paran{ \hbR - \bR\bH_R}^\top
        \cdot \sum_{s=1}^{T} \bE_s \bE_s^\top \bE_t \bC
        +  \frac{1}{p^2 q^2 T} \bH_R^\top \bR^\top  \sum_{s=1}^{T} \bE_s \bE_s^\top \bE_t \bC \\
        & = \frac{1}{p^2 q^2 T} \paran{ \hbR - \bR\bH_R}^\top
        \cdot \sum_{s=1}^{T} \paran{\bE_s \bE_s^\top - \E{\bE_s \bE_s^\top} } \bE_t \bC
        +  \frac{1}{p^2 q^2 T} \paran{ \hbR - \bR\bH_R}^\top
        \cdot \sum_{s=1}^{T} \E{\bE_s \bE_s^\top} \bE_t \bC \\
        & +  \frac{1}{p^2 q^2 T} \bH_R^\top \bR^\top
        \cdot \paran{\bE_s \bE_s^\top - \E{\bE_s \bE_s^\top} } \bE_t \bC
        +  \frac{1}{p^2 q^2 T} \bH_R^\top \bR^\top  \cdot\sum_{s=1}^{T} \E{\bE_s \bE_s^\top} \bE_t \bC \\
        & = {\rm III_1 + III_2 + III_3 + III_4}.
    \end{aligned}
\end{equation}
We bound each term on the right hand side of \eqref{lemma:F_term_2-2} in the sequel.
\begin{equation*}
    \begin{aligned}
        \norm{\rm III_1}
        & \le \frac{1}{p^2 q^2 T}  \norm{ \paran{ \hbR - \bR\bH_R}^\top }
            \cdot \norm{ \sum_{s=1}^{T} \paran{\bE_s \bE_s^\top - \E{\bE_s \bE_s^\top} } \bE_t \bC } \\
        & \le \frac{1}{pq \sqrt{pqT}}
        \cdot  \norm{ \paran{ \hbR - \bR\bH_R}^\top }
        \cdot \norm{ \frac{1}{\sqrt{pqT}} \sum_{s=1}^{T} \paran{\bE_s \bE_s^\top - \E{\bE_s \bE_s^\top} } }
        \cdot \norm{\bE_t \bC}_F  \\
        & =  \frac{1}{\sqrt{q T}}
        \cdot  \frac{1}{\sqrt{p}} \norm{ \paran{ \hbR - \bR\bH_R}^\top }
        \cdot \norm{ \frac{1}{\sqrt{pqT}} \sum_{s=1}^{T} \paran{\bE_s \bE_s^\top - \E{\bE_s \bE_s^\top} } }
        \cdot \paran{ \frac{1}{p} \sum_{i=1}^p \norm{\frac{1}{q}\sum_{j=1}^{q} e_{t,ij} \bC_{j \cdot}}^2 }^{1/2}  \\
         & = \Op{\frac{1}{\delta_{pqT} \sqrt{q T}}},
    \end{aligned}
\end{equation*}
where we use Lemma \ref{assume:moments_Et_0} (a) in the last step.

\begin{equation*}
    \begin{aligned}
        \norm{\rm III_2}
        & = \norm{\frac{1}{p^2 q^2 T} \paran{ \hbR - \bR\bH_R}^\top
            \cdot \sum_{s=1}^{T} \E{\bE_s \bE_s^\top} \bE_t \bC} \\
        & \le  \frac{1}{pq} \cdot \frac{1}{\sqrt{p} }
        \cdot  \frac{1}{\sqrt{p}} \norm{ \paran{ \hbR - \bR\bH_R}^\top }
        \cdot \norm{ \E{ \frac{1}{qT} \sum_{s=1}^{T}  \bE_s \bE_s^\top}}
        \cdot \norm{\bE_t \bC}_F  \\
        & =  \frac{1}{p}
        \cdot  \frac{1}{\sqrt{p}} \norm{ \paran{ \hbR - \bR\bH_R}^\top }
        \cdot \norm{ \E{ \frac{1}{qT} \sum_{s=1}^{T}  \bE_s \bE_s^\top}}
        \cdot \paran{ \frac{1}{p} \sum_{i=1}^p \norm{\frac{1}{q}\sum_{j=1}^{q} e_{t,ij} \bC_{j \cdot}}^2 }^{1/2}  \\
        &=  \Op{\frac{1}{p \delta_{pqT}}},
    \end{aligned}
\end{equation*}
where we use Theorem \ref{thm:Rhat_F_norm_convg} and Lemma \ref{assume:cross_row_col_corr_0}.
\begin{equation*}
    \begin{aligned}
    \norm{\rm III_3}
    & = \frac{1}{p^2 q^2 T} \norm{ \bH_R^\top \bR^\top
        \cdot \sum_{s=1}^{T} \paran{\bE_s \bE_s^\top - \E{\bE_s \bE_s^\top} } \bE_t \bC } \\
    & \le \frac{1}{\sqrt{p q T}}
        \cdot  \norm{ \bH_R^\top }
        \cdot \frac{1}{\sqrt{p}}  \norm{ \bR^\top }
        \cdot \norm{\frac{1}{\sqrt{p q T}}  \sum_{s=1}^{T} \paran{\bE_s \bE_s^\top - \E{\bE_s \bE_s^\top} } }
        \cdot \paran{ \frac{1}{p} \sum_{i=1}^p \norm{\frac{1}{q}\sum_{j=1}^{q} e_{t,ij} \bC_{j \cdot}}^2 }^{1/2} \\
    & =  \Op{ \frac{1}{\sqrt{p q T}}} ,
    \end{aligned}
\end{equation*}
where we use Lemma \ref{assume:moments_Et_0} (a) in the last step.
\begin{equation*}
    \begin{aligned}
        \norm{\rm III_4}
        & = \norm{\frac{1}{p^2 q^2 T} \bH_R^\top \bR^\top  \cdot\sum_{s=1}^{T} \E{\bE_s \bE_s^\top} \bE_t \bC}  \\
        & \le  \frac{1}{p}
        \cdot  \norm{ \bH_R^\top }
        \cdot \frac{1}{\sqrt{p}}  \norm{ \bR^\top }
        \cdot \norm{ \E{ \frac{1}{qT} \sum_{s=1}^{T}  \bE_s \bE_s^\top}}
        \cdot \paran{ \frac{1}{p} \sum_{i=1}^p \norm{\frac{1}{q}\sum_{j=1}^{q} e_{t,ij} \bC_{j \cdot}}^2 }^{1/2}  \\
        &=  \Op{\frac{1}{p}},
    \end{aligned}
\end{equation*}
Finally, we deal with term II in \eqref{eqn:lemma:F_term_2-1}.
Note that
\begin{eqnarray}
{\rm II}& = & \frac{1}{p^2 q^2 T} \sum_{s=1}^{T} \hbR^\top \bR  \bF_s  \bC^\top \bE_s^\top \bE_t \bC \nonumber \\
& = & \frac{1}{p^2 q^2 T} \sum_{s=1}^{T} \left( \hbR - \bR \bH_R \right)^\top \bR  \bF_s  \bC^\top \bE_s^\top \bE_t \bC  + \; \frac{1}{p^2 q^2 T} \sum_{s=1}^{T} \bH_R^\top \bR^\top \bR  \bF_s  \bC^\top \bE_s^\top \bE_t \bC  \nonumber \\
& = & {\rm II_1 + II_2}  \nonumber
\end{eqnarray}
Similar to analysis of term ${\rm III}$, we obtain ${\rm II} = \Op{\frac{1}{ \delta_{pqT}^2}}$.
\end{proof}

\begin{lemma} \label{lemma:E_term}
	Under Assumption \ref{assume:alpha-mixing}-\ref{assume:eigen-val},
	\[
    \frac{1}{p q} \bH_R^\top \bR^\top \bE_t \bC \bH_C = \Op{\frac{1}{\sqrt{pq}}}.
	\]
\end{lemma}
\begin{proof}
    Firstly, by Lemma \ref{assume:moments_Et_0} (b) and Markov inequality, we have $\frac{1}{\sqrt{p q}} \bR^\top \bE_t \bC = \Op{1}$. Combining results in Proposition \ref{thm:bound H}, we have
	\begin{equation*}
	\frac{1}{p q} \bH_R^\top \bR^\top \bE_t \bC \bH_C =  \frac{1}{\sqrt{p q}} \bH_R^\top \paran{  \frac{1}{\sqrt{p q} } \bR^\top \bE_t \bC } \bH_C = \Op{\frac{1}{\sqrt{pq}}}.
	\end{equation*}
\end{proof}

\subsection{Theorem \ref{thm:asymp_St}: Convergence rate of \texorpdfstring{$\hat \bS_t$}{hat S}}  \label{sec:proof S_t}

\paragraph{Proof of Theorem \ref{thm:asymp_St}.}
Define $\tbR_{i \cdot} = \bH_R^\top \bR_{i \cdot}$, $\tbC_{j \cdot} = \bH_C^\top \bC_{j \cdot}$, and $\tbF_t = \bH_R^{-1} \bF_t {\bH_C^\top}^{-1}$, we have

\begin{equation*}
    \begin{aligned}
        \hat \bS_{t,ij} - \bS_{t,ij}
        & =  \hbR_{i \cdot}^\top \hbF_t \hbC_{j \cdot} - \bR_{i \cdot}^\top \bF_t \bC_{j \cdot}
            = \hbR_{i \cdot}^\top \hbF_t \hbC_{j \cdot} - \tbR_{i \cdot}^\top \tbF_t \tbC_{j \cdot}  \\
        & =  \left( \hbR_{i \cdot} - \tbR_{i \cdot} \right)^\top \left( \hbF_t - \tbF_t \right) \left( \hbC_{j \cdot} - \tbC_{j \cdot} \right)  \\
        &     + \left( \hbR_{i \cdot} - \tbR_{i \cdot} \right)^\top \tbF_t \left( \hbC_{j \cdot} - \tbC_{j \cdot} \right)
               + \;  \tbR_{i \cdot}^\top \left( \hbF_t - \tbF_t \right) \left( \hbC_{j \cdot} - \tbC_{j \cdot} \right)
               + \left( \hbR_{i \cdot} - \tbR_{i \cdot} \right)^\top \left( \hbF_t - \tbF_t \right) \tbC_{j \cdot}  \\
        &  + \; \tbR_{i \cdot}^\top \tbF_t \left( \hbC_{j \cdot} - \tbC_{j \cdot} \right)
            + \left( \hbR_{i \cdot} - \tbR_{i \cdot} \right)^\top \tbF_t \tbC_{j \cdot}
            + \tbR_{i \cdot}^\top \left( \hbF_t - \tbF_t \right) \tbC_{j \cdot} .
    \end{aligned}
\end{equation*}
Dominant terms are the last three terms.
Note that $\norm{\tilde\bF_t} = \Op{1}$, $\norm{\tbC_{j \cdot}} = \Op{1}$ and $\norm{\tbR_{i \cdot}^\top} = \Op{1}$.
From Theorem \ref{thm:asymp normality of R/C}, we have
\[
\hbR_{i \cdot} - \tbR_{i \cdot} = \Op{\frac{1}{\min \paran{p, \sqrt{qT}} }}, \quad \text{and    } \hbC_{j \cdot} - \tbC_{j \cdot} = \Op{\frac{1}{\min \paran{q, \sqrt{pT}} }}.
\]
Then using Theorem \ref{thm:asymp_Ft}, we have
\[
\hat \bS_{t,ij} - \bS_{t,ij} = \Op{\frac{1}{\min \paran{p, q, \sqrt{qT}, \sqrt{pT}}}}.
\]

%\input{consist-k.tex}

\subsection{Theorem \ref{thm:cov-est-consistent}: Consistent covariance estimators}  \label{sec:proof_cov_est_consistent}
%\noindent\textbf{Proof of Theorem \ref{thm:cov-est-consistent}}

\begin{proof}
In the following, we show that under Assumption A-G and uncorrelated rows and columns, as $p$, $q$, $T \longrightarrow \infty$, $\hat \bSigma_{R_i}$ is consistent for $\bSigma_{R_i}$. Proof for $\hat \bSigma_{C_j}$ is similar.

It suffice to prove that the HAC estimator based on estimators $\{ \hat \bF_t \hat \bC^\top \hat \be_{t, i \cdot} \}_{t = 1, \ldots, T}$, that is
\[
\hat \bGamma_R \; \defeq \; \bD_{R, 0,i} + \sum_{\nu = 1}^{m} \paran{1 - \frac{\nu}{1 + m}} \paran{\bD_{R, \nu, i} + \bD_{R, \nu, i}^\top},
\]
is a consistent estimator of $\bQ_R \bPhi_{R, i} \bQ_R^\top$.

Because $\hat \bF_t$ estimates $\bH_R^{-1} \bF_t {\bH_C^\top}^{-1}$ and $\hat \bC$ estimates $\bC \bH_C$, the HAC estimator $\hat \bGamma_R$ is estimating $\bH_R^{0, -1} \bPhi_{R, i} {\bH_R^{0, -1}}^\top$ where $\bH_R^{0}$ is the limit of $\bH_R$ \citep{newey1987simple}. Recall that
\[
\bH_R = \frac{1}{p q T} \sum_{t=1}^{T} \bF_t \bC^\top \bC \bF_t^\top \bR^\top \hat \bR \bV_{R, pqT}^{-1}  \convprob \bSigma_{FC} \bQ_R^\top \bV_R^{-1},
\]
and $\norm{\bH_R} = \Op{1}$ and $\norm{\bH_R^{-1}} = \Op{1}$.
By Proposition \ref{prop:RhatR}, we further have,
\[
\bSigma_{FC} \bQ_R^\top \bV_R^{-1} = \bSigma_{FC} \paran{\bV_R^{1/2} \; \bPsi_R^\top \; \bSigma_{FC}^{- 1/2}}^\top \bV_R^{-1} = \bSigma_{FC}^{1/2} \; \bPsi_R \; \bV_R^{-1/2}  = \bQ_R^{-1},
\]
where we use the fact that $\bPsi_R^\top \bPsi_R = \bI$.
Thus, $\hat \bGamma_R$ consistently estimates $\bQ_R \bPhi_{R, i} \bQ_R^\top$.
\end{proof}







